Bi-CL: A Reinforcement Learning Framework for Robots Coordination Through Bi-level Optimization

In multi-robot systems, achieving coordinated missions remains a significant challenge due to the coupled nature of coordination behaviors and the lack of global information for individual robots. To mitigate these challenges, this paper introduces a novel approach, Bi-level Coordination Learning (Bi-CL), that leverages a bi-level optimization structure within a centralized training and decentralized execution paradigm. Our bi-level reformulation decomposes the original problem into a reinforcement learning level with reduced action space, and an imitation learning level that gains demonstrations from a global optimizer. Both levels contribute to improved learning efficiency and scalability. We note that robots' incomplete information leads to mismatches between the two levels of learning models. To address this, Bi-CL further integrates an alignment penalty mechanism, aiming to minimize the discrepancy between the two levels without degrading their training efficiency. We introduce a running example to conceptualize the problem formulation and apply Bi-CL to two variations of this example: route-based and graph-based scenarios. Simulation results demonstrate that Bi-CL can learn more efficiently and achieve comparable performance with traditional multi-agent reinforcement learning baselines for multi-robot coordination.

==> Contents_backup/abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{abstract}
    In multi-robot systems, achieving coordinated missions remains a significant challenge due to the coupled nature of coordination behaviors and the lack of global information for individual robots.
    To mitigate these challenges, this paper introduces a novel approach, Bi-level Coordination Learning (Bi-CL), that leverages a bi-level optimization structure within a centralized training and decentralized execution paradigm. Our bi-level reformulation decomposes the original problem into a reinforcement learning level with reduced action space, and an imitation learning level that gains demonstrations from a global optimizer. Both levels contribute to improved learning efficiency and scalability. We note that robots' incomplete information leads to mismatches between the two levels of learning models. To address this, Bi-CL further integrates an alignment penalty mechanism, aiming to minimize the discrepancy between the two levels without degrading their training efficiency. We introduce a running example to conceptualize the problem formulation and apply Bi-CL to two variations of this example: route-based and graph-based scenarios. Simulation results demonstrate that Bi-CL can learn more efficiently and achieve comparable performance with traditional multi-agent reinforcement learning baselines for multi-robot coordination. 



    
    %Bi-CL not only enhances learning efficiency but also maintains the intricate cooperative relationships between the execution of individual actions and group coordination behaviors. 
    
    
    %To mitigate the gap between the two levels of bi-level optimization due to incomplete information, Bi-CL further integrates an alignment penalty as a bridge between the two levels, aiming at minimizing the discrepancy and fostering better coordination and efficiency. We introduce a running example to conceptualize the problem formulation and apply Bi-CL to two variations of this example: route-based and graph-based scenarios. Simulation results demonstrate that Bi-CL can more efficiently learn and achieve comparable performance with traditional multi-agent reinforcement learning baselines for multi-robot coordination. 

    %To address these challenges, this paper introduces a novel approach, Bi-level Coordination Learning (Bi-CL).
    %Bi-CL is enabled by a bi-level optimization reformulation of multi-robot coordination within a centralized training and decentralized execution paradigm. One level of the problem is composed of a 
    
\end{abstract}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Contents_backup/approach.tex <==
\section{Main Approach}
%\marginXW{Worked till here}
%\subsection{CDET: Reinforcement learning + Imitation learning} 

%Given the characteristics \ref{eq_trans} \ref{eq_rew} of our formulation, it is evident that for each state transition, we need to optimize the discrete action to achieve the maximum reward under the known current state and the selected continuous action. Consequently, for the decision-making regarding the discrete action, upon knowing $\bm{s}^t$ and $\bm{a}_1^t$ at every step, incorporating a discrete optimizer, such as enumeration, dynamic programming, or greedy algorithms, enables us to find the optimal combination of $\bar{\bm{a}_2}^t$ under the given moment and conditions, which reads
%\begin{align}
%    \bar{\bm{a}_2}^t = f(\bm{s}^{t+1}) = f(\bm{s}^t, \bm{a}_1^t, \mathcal{T})
%\end{align}
%where, $\bar{\bm{a}_2}^t$ represents the optimal discrete action combination for the team, $f$ represents the discrete optimizer here. 

%By integrating a Discrete Optimizer, it effectively transforms the original multi-agent system from a two-dimensional hybrid action space into a one-dimensional continuous action space, which significantly enhances the efficiency of subsequent policy learning processes.

 %To address this, our idea is to train two local policies $$

%assumes the availability of global information. When implementing a decentralized approach, we encounter the challenge that each agent relies on local observations ${{s}}^{\mathcal{N}_i}_t \subsetneq {\bm{s}}_t$ to decide its actions. 
%We can employ a similar two-step mechanism, which first uses reinforcement learning to learn a local policy $\widehat \pi^i: \mathcal{S}^{\mathcal{N}_i}\to {\mathcal{X}}^i$ to determine ${\bm{x}}_t^i$ for each agent. However, in the second step, the local observation prohibits us from using an optimizer to generate the action ${\bm{y}}_t^i$ because it relies on global state and global action. %To address this, a feasible approach is to introduce another layer of reinforcement learning model to determine  $\widehat \eta^i: \mathcal{S}^{\mathcal{N}_i}\times {\mathcal{X}}^{\mathcal{N}_i}\to {\mathcal{Y}}^i$. However, since the global reward, c.f. \eqref{eq_rew_c}, rely on both action ${\bm{x}}_t,{\bm{y}}_t$, using two layers of coupled reinforcement learning results in poor convergence stability and low learning efficiency [x]. In some cases, it may even be less desirable than using reinforcement learning to learn ${\bm{x}}_t,{\bm{y}}_t$ simultaneously. 
%we will leverage the hierarchical action structure of the problem, and introduce a new approach (cf. Fig.\ref{fig_dist_optimizer}). The approach uses a reinforcement learning mechanism to determine $\widehat{\pi}^i$, and an imitation learning mechanism to learn a policy $\widehat \eta^i: \mathcal{S}^{\mathcal{N}_i}\times {\mathcal{X}}^{\mathcal{N}_i}\to {\mathcal{Y}}^i$. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{Figures/method/Algorithm_D.pdf}
  \caption{A Bi-level Coordination Learning (Bi-CL) Algorithm: incorporating multi-agent reinforcement learning (MARL) and imitation learning (MAIL), guided by a global optimizer.}
   \label{fig_dist_optimizer}
\end{figure}

As described in Sec. \ref{sec_centralized_bi}, the centralized bi-level formulation leverages the optimizer \eqref{eq_opt_bara} to reduce the dimensionality of the action space, thereby enhancing training efficiency. However, such optimization requires global information, which is not accessible to robots during decentralized execution. Thus, robots cannot locally generate ${y_t^i}^{*}$.
To address this issue, in this section, we introduce a new reformulation to generalize the concept of bi-level optimization to a CTDE  setup. %{\color{red}[Add description of novelty?]}

%our approach employs a similar two-step mechanism and trains two local policies for each robot: one policy, $\widehat{\pi}^i: \mathcal{S}^{\mathcal{N}_i} \to \mathcal{X}^i$, generates $x^i_t$; another policy, ${\eta}^i: \mathcal{S}^{\mathcal{N}_i} \times \mathcal{X}^{\mathcal{N}_i} \to \mathcal{Y}^i$, generates actions $y^i_t$. We employ CTDE (Centralized Training with Decentralized Execution). With the help of a global optimizer, $\widehat{\pi}^i$ is trained using reinforcement learning with a reduced-action space. ${\eta}^i$ is trained using imitation learning, taking the global optimizer as an expert demonstration. Since the parameters of the two models are trained separately, we further introduce a penalty mechanism in the optimizer to ensure the alignment of the two policies.

To present our approach, we reformulate \eqref{eq_loca_prob} into the following Bi-level Coordination Learning (Bi-CL) problem, $\forall i\in\{1,\cdots,n\}$,
\begin{subequations}\label{eq_d_prob2}
    \begin{align}\label{eq_bilevel_d}
    &\max_{\widehat\pi^i} \quad\underset{{x}^i_t \sim \widehat\pi^i(\cdot|{s}^{\mathcal{N}_i}_t)}{\mathbb{E}}\left[\sum_{t=0}^T \gamma^t U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t))\right], 
    \\
    %&\min_{\eta^i} \quad\underset{{y}^i_t \sim \eta^i(\cdot|{s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)}{\mathbb{E}}\left[\mathcal{D}\big({y}^i_t,{{y}^i_t}^*(\bm{s}_t,{\bm{x}}_t)\big)\right]\label{eq_policy_bara_d}
    &\min_{\eta^i} \quad\underset{{y}^i_t \sim \eta^i(\cdot|{s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)}{\mathbb{E}}\|{y}^i_t - {{y}^i_t}^*(\bm{s}_t,{\bm{x}}_t)\|^2\label{eq_policy_bara_d}, 
    \\
    &\text{s.t.}~ {\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t)\!=\! \arg\max_{{\bm{y}}_t}\!\left[U({\bm{s}}_t\!,{\bm{x}}_t\!,{\bm{y}}_t) 
    \underbrace{-c_k \sum_{i=1}^{n}\mathcal{H}_i({y}^i_t, \eta^i))}_{\text{alignment penalty}}\right] \label{eq_opt_bara_d}
\end{align}
\end{subequations}
In equations \eqref{eq_bilevel_d} and \eqref{eq_policy_bara_d}, we aim to train two local policies for each robot: one policy, $\widehat{\pi}^i: \mathcal{S}^{\mathcal{N}_i} \to \mathcal{X}^i$, generates action $x^i_t$; another policy, ${\eta}^i: \mathcal{S}^{\mathcal{N}_i} \times \mathcal{X}^{\mathcal{N}_i} \to \mathcal{Y}^i$, generates action $y^i_t$.
Note that the two policies are coupled since their inputs rely on the outputs of each other. If training two policies simultaneously, such coupling can pose a stability issue and reduce training efficiency. To address this, our idea is to introduce a global optimizer \eqref{eq_opt_bara_d} under the CTDE scheme to decouple and guide the training of both policies, as we explain next and visualized in Fig. \ref{fig_dist_optimizer}.

%Firstly, equations \eqref{eq_bilevel_d} and \eqref{eq_opt_bara_d} represent a CTDE version of the bi-level problem \eqref{eq_c_prob2}. Temporarily ignore the penalty term. We introduce optimization problem \eqref{eq_opt_bara_d} to solve ${\bm{y}}_t^{\star}$. This solution is only used during the centralized training process and thus can utilize global information by aggregating all robots' states ${\bm{s}}_t$ and actions ${\bm{x}}_t$. Based on ${\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t))$, we train the local policy $\widehat\pi^i$ in \eqref{eq_bilevel_d} for each agent's ${{x}}^i_t$ using a \textit{reinforcement learning} scheme over a \textit{reduced-dimension} action space. 

\noindent\textbf{Bi-level optimization:} First, we introduce optimization problem \eqref{eq_opt_bara_d} to solve ${\bm{y}}_t^{\star}$. If temporarily ignoring the alignment penalty term, the equations \eqref{eq_bilevel_d} and \eqref{eq_opt_bara_d} together represent a CTDE version of the bi-level problem \eqref{eq_c_prob2}.  During the centralized training process, we can utilize global information for all robots' states ${\bm{s}}_t$ and actions ${\bm{x}}_t$ to solve ${\bm{y}}_t^{\star}$. Based on ${\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t)$, we train the local policy $\widehat\pi^i$ in \eqref{eq_bilevel_d} for each agent's ${{x}}^i_t$ using a \textit{reinforcement learning} scheme. $\widehat\pi^i$ has a \textit{reduced-dimension} action space because ${\bm{y}}_t^{\star}$ is not learned. 

On the other hand, while optimizer \eqref{eq_opt_bara_d} can be used in centralized training to obtain action ${\bm{y}}_t^{\star}$ for all robots, it cannot be used by robots during decentralized execution due to the local observations. Thus, we introduce \eqref{eq_policy_bara_d} to train a local policy $\eta^i$ to generate agent's ${{y}}^i_t$. The policy $\eta^i$ can be trained conveniently using an imitation learning (IL) scheme that uses optimizer \eqref{eq_opt_bara_d} as the \textit{expert demonstration}. 
%Here, a possible choice for the imitation loss $\mathcal{D}$ is 
%$$\mathcal{D}=\|{y}^i_t - {{y}^i_t}^*(\bm{s}_t,{\bm{x}}_t)\|,$$ 
Here, the imitation loss in \eqref{eq_policy_bara_d} measures the difference between the policy output ${y}^i_t$ using local information and the optimal action solved from optimizer \eqref{eq_opt_bara_d} using global information.


\begin{algorithm2e}[t]
\SetAlgoLined
% \KwResult{Trained Actor and Critic Networks}
 \textbf{Initialize} local RL models $\widehat{\pi}^i({s}^{\mathcal{N}_i}|\theta_{\widehat{\pi}^i})$ and IL models $\eta^i({s}^{\mathcal{N}_i}, x^{\mathcal{N}_i}|\theta_{\eta^i})$ for all robots. Initialize centralized critic $Q(\bm{s}, \bm{x}|\theta_Q)$ if needed;  \\
 \textbf{Initialize} alignment penalty co-efficient $c_k$;\\
 %\textbf{Initialize} step-size $\delta$ and replay buffer $\mathcal{B}$; \\
 %\textbf{Initialize} target networks $Q'$ and $\widehat{\pi}^{i'}$ with weights $\theta^{Q'} \leftarrow \theta^Q$ and $\theta^{\widehat{\pi}^{i'}} \leftarrow \theta^{\widehat{\pi}^i}$;\\
 \For{$\text{k} = 0$ \KwTo $T_k$}{
  %\textbf{Initialize} a random process $\mathcal{D}$, receive initial global state $\bm{s}_1$ and local observations ${\bm{s}}^{\mathcal{N}_i}_1$;\\
    Update coefficient $c_k=\frac{c}{1+e^{-\beta (k-h)}}$;\\
  \For{$t = 0$ \KwTo $T_t$}{
  \For{$i = 1$ \KwTo $n$}{
  Get action: $x^i_t$ by adding random perturbation to ${\widehat{\pi}^i}({s}^{\mathcal{N}_i}_t|\theta_{\widehat{\pi}^i})$;\\
   %Execute $x^i_t$;\\
   Get action: $\widehat{y}^i_t = \eta^i({s}^{\mathcal{N}_i}_t,{x}^i_t | \theta_{\eta^i})$;\\
   State update: ${s}^i_{t+1}=\mathcal{T}^i({s}^i_t, {x}^i_t)$;\\
   }
   Solve $\arg\max_{{\bm{y}}_t}\!\left[U(\bm{s}_t, \bm{x}_t, \bm{y}_t) 
    -c_k \sum_{i=1}^n\mathcal{H}_i\right]$ to obtain ${\bm{y}}_t^{\star}$;\\
   Observe reward $R_t = U(\bm{s}_t, \bm{x}_t, \bm{y}_t^{\star});$\\
   Record $(\bm{s}_t, \bm{x}_t, \bm{y}^{\star}_t, R_t, \bm{s}_{t+1})$ to a fixed size buffer $\mathcal{B}$ with first-in-first-out;\\
   Sample $(\bm{s}_{\tau}, \bm{x}_{\tau}, \bm{y}^{\star}_{\tau}, r_{\tau}, \bm{s}_{{\tau}+1})$ from $\mathcal{B}$ as a random minibatch of size $w$;\\
   Update critic network $\theta_{Q}$ using the minibatch, if critic exist;\\
   \For{$i = 1$ \KwTo $n$}{
    Update IL learning model $\theta_{\eta^i}$ using the minibatch;\\
    Update RL learning model: $\theta_{\widehat{\pi}^i}$ using the minibatch;
   }
   %Update each target network:\\
   %$\theta^{Q'} \leftarrow \tau\theta^Q + (1 - \tau)\theta^{Q'}$;\\
   %$\theta^{\widehat{\pi}^{i'}} \leftarrow \tau\theta^{\widehat{\pi}^{i}} + (1 - \tau)\theta^{\widehat{\pi}^{i'}}$;\\
  }
 }
 \caption{{The Bi-CL Algorithm}}
 \label{alg_1}
\end{algorithm2e}

\noindent\textbf{Alignment of the two policies:} We explain the alignment term in \eqref{eq_opt_bara_d}. Based on the above explanation, the policy $\widehat\pi^i$ is trained assuming the actions ${\bm{y}}_t^{\star}=\{{y^1_t}^*,\cdots,{y^n_t}^*\}$ are optimal for all robots, and the policy $\eta^i$ seeks to generate such optimal actions using only local information. Clearly, during decentralized execution, the optimality of $\eta^i$ can hardly be guaranteed, thus creating a mismatch between the policies $\widehat\pi^i$ and $\eta^i$. To address this, we introduce an alignment penalty term $c_k \sum_{i=1}^{n}\mathcal{H}_i({y}^i_t, \eta^i))$ in \eqref{eq_opt_bara_d}, where $c_k>0$ and
%$$\mathcal{H}_i=\|{y}^i_t-\mathbb{E}[\eta^i({s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)] \|$$ 
$$\mathcal{H}_i=\underset{\widehat{y}^i_t \sim \eta^i(\cdot|{s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)}{\mathbb{E}}\|{y}^i_t - {\widehat{y}^i_t}\|^2.$$ 
%\marginZC{$\widehat{y}^i_t=\eta^i(\cdot|{s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)$, ${\widehat{y}^i_t}$ is from the model}
Here, ${\widehat{y}^i_t}$ is the output of the model $\eta^i$, then $\mathcal{H}_i$ evaluates how well an action ${y}^i_t$ aligns with the policy $\eta^i$. Minimizing this penalty helps to reduce the mismatch between the two local policies. Mathematically, the value of $\mathcal{H}_i$ for each robot equals the loss in \eqref{eq_policy_bara_d}. Hence, $c_k$ is an important coefficient and we shall remark on its choice during the training. If $c_k \to 0$, the reformulation \eqref{eq_d_prob2} disregards the policy mismatch, always opting for the solution that maximizes $U$ to train $\widehat\pi^i$. 
Conversely, when $c_k\to \infty$, the penalty forces the training of $\widehat\pi^i$ using the action chosen by $\eta^i$, making the two policies fully coupled, and the IL \eqref{eq_policy_bara_d} no longer updates. 
To strike a balance, our idea is to make sure the IL model is sufficiently trained before the penalty is applied. For this purpose, we define a modified logistic function:
\begin{align}\label{eq_defck}
    c_k=\frac{c}{1+e^{-\beta (k-h)}}\quad \text{with}\quad c>0, \beta>0, h>0
\end{align}
where $k$ is the training episode. We let $c_k$ start with zero to `jump start' the training of $\widehat\pi^i$ and $\eta^i$ using the optimal ${\bm{y}}_t^{\star}$ for maximizing $U$. Afterwards, $c_k$ is gradually increased to a sufficiently large value $c$ to fine-tune $\widehat\pi^i$, taking into account the output of $\eta^i$ and ensuring alignment between the two policies, $\widehat\pi^i$ and $\eta^i$.
The described training scheme is summarized in Algorithm 1. 

% \begin{algorithm}[H]
% \SetAlgoLined
% % \KwResult{Trained Actor and Critic Networks}
% \textbf{Initialize} critic $Q(s, x, y|\theta^Q)$, actors $\widehat{\pi}^i(s|\theta^{\widehat{\pi}^i})$, target networks $Q'$, $\widehat{\pi}^{i'}$, replay buffer $R$, datasets $D^i$;\\
% \For{$\text{episode} = 1$ \KwTo $M$}{
%   Initialize random process $\mathcal{N}$, receive initial state $s_1$ and observations ${s}^{\mathcal{N}_i}_1$;\\
%   \For{$t = 1$ \KwTo $T$}{
%     \For{$i = 1$ \KwTo $n$}{
%       Select $x^i_t = {\widehat{\pi}^i}({s}^{\mathcal{N}_i}_t|\theta^{\widehat{\pi}^i}) + \mathcal{N}_t$, execute $x^i_t$, observe new state $s_{t+1}$, ${s}^{\mathcal{N}_i}_{t+1}$, reward $r_t$;\\
%     }
%     Store $(s_t, x_t, r_t, s_{t+1})$ in $R$, sample minibatch from $R$, compute target $y_j$, update critic, update actors, update target networks;\\
%   }
% }
% \For{$i = 1$ \KwTo $n$}{
%     \For{each data point in $D^i$}{
%         Construct $\eta_i$ using ${s}^{\mathcal{N}_i}_t, x^i_t$ to predict ${y^i_t}^*$:\\
%         \Indp Initialize $\eta_i$, determine best split, split dataset, recursively build tree, label leaves;\\
%         \Indm Evaluate $\eta_i$ on validation set;\\
%     }
% }
% \caption{Simplified DDPG and Decision Tree Training}
% \end{algorithm}

%\marginXW{what is $s_{\tau+1}$}
%\marginXW{Orders?}
%\marginXW{minibatch, where loops end?}
%\marginXW{why $Q'$}

\begin{comment}
\begin{algorithm}
\SetAlgoLined
% \KwResult{Trained Actor and Critic Networks}
 \textbf{Initialize} centralized critic $Q(s, x, y|\theta^Q)$, local actors $\widehat{\pi}^i({s}^{\mathcal{N}_i}|\theta^{\widehat{\pi}^i})$ and local policies $\eta^i({s}^{\mathcal{N}_i}, x^i|\theta^{\eta^i})$ for all robots \\
 \textbf{Initialize} coefficients $c_k=c(1-e^{-\beta t})$ and replay buffer $\mathcal{B}$; \\
 %\textbf{Initialize} target networks $Q'$ and $\widehat{\pi}^{i'}$ with weights $\theta^{Q'} \leftarrow \theta^Q$ and $\theta^{\widehat{\pi}^{i'}} \leftarrow \theta^{\widehat{\pi}^i}$;\\
 \For{$\text{episode} = 1$ \KwTo $T_e$}{
  \textbf{Initialize} a random process $\mathcal{D}$, receive initial global state $\bm{s}_1$ and local observations ${\bm{s}}^{\mathcal{N}_i}_1$;\\
  \For{$t = 1$ \KwTo $T$}{
  \For{$i = 1$ \KwTo $n$}{
   Select action $x^i_t = {\widehat{\pi}^i}({s}^{\mathcal{N}_i}_t|\theta^{\widehat{\pi}^i}) + \mathcal{N}_t$;\\
   Execute $x^i_t$;\\
   Get action $\widehat{y}^i_t = \eta^i({s}^{\mathcal{N}_i}_t,{x}^i_t | \theta^{\eta^i})$
   }
   Receive $(\bm{s}_{t+1}, {\bm{s}}^{\mathcal{N}_i}_{t+1})=\mathcal{T}(\bm{s}_t, \bm{x}_t)$;\\
   ${\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t)\!=\! \arg\max_{{\bm{y}}_t}\!\left[U({\bm{y}}_t|{\bm{s}}_t,{\bm{x}}_t) 
    -c_k \sum_{i}\mathcal{H}_i\right]$;\\
   Receive optimal $\bm{y}_t$ combinations;\\
   Observe reward $r_t = U(\bm{s}_t, \bm{x}_t, \bm{y}_t^{\star})$\\
   Add $(\bm{s}_t, \bm{x}_t, \bm{y}^{\star}, r_t, \bm{s}_{t+1})$ to $\mathcal{B}$;\\
   Sample a random minibatch $(\bm{s}_{\tau}, \bm{x}_{\tau}, \bm{y}^{\star}, r_{\tau}, \bm{s}_{{\tau}+1})$ with size $W$ from $R$;\\
   \For{$i = 1$ \KwTo $n$}{
   Update each {\color{blue}optimizer policy} by minimizing the sample {\color{blue}optimizer policy} loss:\\
    $L^i_{{\color{blue}optimizer}} = - \frac{1}{W}\sum_{{\tau}} (y_{\tau}^{i\star}-\eta^i({s}^{\mathcal{N}_i}_{\tau},{x}^i_{\tau} | \theta^{\eta^i}))^2$
   }
   Set $z_{\tau} = r_{\tau} + \gamma Q'(\bm{s}_{{\tau}+1}, \bm{x}_{{\tau}+1}|\theta^{Q'})$ where $x^i_{{\tau}+1} = \widehat{\pi}^{i'}({s}^{\mathcal{N}_i}_{{\tau}+1}|\theta^{\widehat{\pi}^{i'}})$;\\
   Update critic by minimizing the critic loss where $L_{\text{critic}} = \frac{1}{W} \sum_{\tau} (z_{\tau} - Q(\bm{s}_{\tau}, \bm{x}_{\tau}|\theta^Q))^2$;\\
   \For{$i = 1$ \KwTo $n$}{
   Update each actor policy using the sampled policy gradient:\\
       $\nabla_{\theta^{\widehat{\pi}^i}} J \approx \frac{1}{N} \sum_{\tau} \nabla_{x_i} Q(\bm{s}, \bm{x}|\theta^Q)\nabla_{\theta^{\widehat{\pi}^i}} \widehat{\pi}^i({s}^{\mathcal{N}_i}|\theta^{\widehat{\pi}^i})|_{{s}^{\mathcal{N}_i}_{\tau}}$\\
    where in $Q(\bm{s}, \bm{x}|\theta^Q)$, ${\bm{s}=\bm{s}_{{\tau}}, x^i=\widehat{\pi}({s}^{\mathcal{N}_i}_{\tau})}$
   }
   Update each target network:\\
   $\theta^{Q'} \leftarrow \tau\theta^Q + (1 - \tau)\theta^{Q'}$;\\
   $\theta^{\widehat{\pi}^{i'}} \leftarrow \tau\theta^{\widehat{\pi}^{i}} + (1 - \tau)\theta^{\widehat{\pi}^{i'}}$;\\
  }
 }
 \caption{{Alg Name}}
\end{algorithm}
\end{comment}

\begin{remark}
    In the presentation of Algorithm \eqref{alg_1}, we assume the use of actor-critic-based methods for \eqref{eq_bilevel_d} and a quadratic mismatch function for the imitation loss \eqref{eq_policy_bara_d}. However, the proposed algorithm is also applicable to general CTDE setups when using other reinforcement learning and imitation learning methods. Furthermore, in handling the local observations of robots, there exist more advanced methods \cite[Sec. 2.2.2]{zhang2021multi} in the literature on Dec-MDPs and POMDPs that leverage the memory (historic states) of robots to learn more powerful policies. In this paper, we only use simple memory-less policies, but these more advanced methods are also compatible with Algorithm \eqref{alg_1}.
\end{remark}

% \begin{algorithm2e}
%     \caption{XXX Algorithm}
%     \label{Alg_XXX}
%     \SetAlgoLined
%     Randomly \textbf{Initialize} critic network $Q(s, \widehat{a}, \bar{a}|\theta^Q)$ and actors $\mu_{i}(s|\theta^{\mu_{i}})$ with weights $\theta^Q$ and $\theta^{\mu_{i}}$;\\
%     \textbf{Initialize} target networks $Q'$ and $\mu_{i}'$ with weights $\theta^{Q'} \leftarrow \theta^Q, \theta^{\mu_{i}'} \leftarrow \theta^{\mu_{i}}$;\\
%     \textbf{Initialize} replay buffer $R$;\\
%     \textbf{Initialize} dataset $D^i$;\\
%     \For{episode = 1, M}{
%     \textbf{Initialize} a random process $\mathcal{N}$ for action exploration;\\
%     Receive initial global state $s_1$;\\
%     \For{t = 1, T}{
%     \For{i \in [1, n]}{
%     Select action $\widehat{a^it} = \mu(o^it|\theta^{\mu_{i}}) + \mathcal{N}_t$ according to the current policy and exploration noise;\\
%     Execute action $\widehat{a^it}$ and explore all possible $\bar{a^i}$ combinations;\\}
%     Observe reward $r_t$ and observe new global state $s_{t+1}$ and return the optimal combination $\bar{\bm{a}^i}$;\\
%     Store transition $(\bm{s}_t, \widehat{\bm{a}_t}, r_t, \bm{s}_{t+1})$ in $R$\;\\
%     Store data $(o^it, \widehat{a^it}, o_{t+1}, \bar{a^it})$ in $D^i$;\\
%     Sample a random minibatch of $N$ transitions $(\bm{s}_t, \widehat{\bm{a}_t}, r_t, \bm{s}_{t+1})$ from $R$;\\
%     \For{each sampled transition}{
%     Set $y_j = r_j + \gamma Q'(\bm{s}_{j+1}, \mu_1'(o_1_{j+1}, |\theta^{\mu_1'}), \mu_2'(o_2_{j+1}, |\theta^{\mu_2'}), \dots, \mu_n'(o_n_{j+1}, |\theta^{\mu_n'})|\theta^{Q'})$;\\
%     }
%     Update critic by minimizing the loss: $L = \frac{1}{N} \sum_j (y_j - Q(\bm{s}_j, \widehat{\bm{a}_j}|\theta^Q))^2$;\\
%     Update each actor policy using the sampled policy gradient:;\\
%     $\nabla_{\theta^{\mu^i}} J \approx \frac{1}{N} \sum_j \nabla_{\widehat{a}} Q(\bm{s}, \widehat{\bm{a}}|\theta^Q)|_{s=\bm{s}_j,\widehat{a}=\mu^i(o^ij)} \nabla_{\theta^\mu} \mu(s|\theta^\mu)|_{s_j}$;\\
%     }
%     }
% \end{algorithm2e}



%once ${\bm{x}}_t$ are determined, we can still utilize the optimizer $f: \mathcal{S}\times {\mathcal{X}}\to\bar{\mathcal{A}}$ to generate the team's optimal combination of the action ${\bm{y}}_t$. 


%As a consequence, we can not only learn a policy $\widehat \pi^i: \mathcal{S}\to {\mathcal{X}}$ for each agent to first determine action ${\bm{x}}_t$, then use an optimizer $f: \mathcal{S}\times {\mathcal{X}}\to\bar{\mathcal{A}}$ to generate the action ${\bm{y}}_t$

%despite the communication barriers between agents, each agent's local observations are aggregated at a central processor. At this point, an optimizer is incorporated at the central unit to generate the team's optimal combination of the discrete action $\bm{a}_2$, which is then disseminated to the respective agents. Consequently, each agent's continuous action $\bm{a}_1$ is produced by its corresponding actor network, while $\bm{a}_2$ are allocated by the optimizer at the central processor. These behaviors are utilized to compute the reward for an actor-critic learning update process. 

%Within this framework, a 'policy' mechanism is introduced. Each agent is assigned a 'policy', which learns, through supervised learning, the agent's optimal $\bm{a}_2$ choice under varying local observations. These 'policies' form the intermediary layer of our learning architecture.

%During decentralized execution, although the central processor is no longer available, each agent can derive its $\bm{a}_1$ from its own actor network. Additionally, the agent is informed of the $\bm{a}_2$ choice it should make by its 'policy', thus facilitating the progression of the Markov Process.

%Such an architecture enables action dimensionality reduction even under conditions of communication constraints.




% \subsection{Local Observation}

% The locality of observation needs to be considered due to multi-agent communication barriers. 

% Let $\delta_{ij}$ be the distance of $i$-th agent and $j$-th agent. Define $\Delta$ as the maximum distance for perfect communication between agents, such that if $\delta_{ij} \leq \Delta$, the state information of agents $i$ and $j$ can be communicated effectively, implying that agents $i$ and $j$ are aware of each other's position. Conversely, if $\delta_{ij} > \Delta$, communication between agents $i$ and $j$ is not possible, leading to a complete lack of state information exchange when the distance exceeds this threshold.

% In a multi-agent system, let $s_j^t$ represent the state of the $j$-th agent at time $t$. Then, the local observation of agent $i$, denoted as $o^i$, at time $t$ is defined by the set:
% \[
% o^i = \{ p_{ij} \cdot s_j^t | 1 \leq j \leq n \}
% \]
% where
% \[
% p_{ij} = \begin{cases} 
% 1 & \text{if } \delta_{ij} \leq \Delta, \\
% 0 & \text{otherwise}.
% \end{cases}
% \]

% \subsection{Optimizer}

% In the formulation, we define the action 'guard' as a team coordination behavior. Due to the presence of cooperative decision-making behavior, our action space is characterized as a hybrid one, encompassing both continuous and discrete domains. Specifically, the velocity behavior $v^i^t$ denotes the speed of the $i$-th agent at time $t$ in the continuous domain, while the guard behavior $g^i^t$ in the discrete domain represents the adversary guarded by the $i$-th agent at time $t$.

% In our MDP model, state transitions, denoted by $\bm{s}_{t+1}$, depend solely on the agents' velocity behaviors $\bm{v}^t$. However, the rewards, $\bm{r}(\bm{s}^t, \bm{a}^t)$, are determined by both velocity $\bm{v}^t$ and guard behaviors $\bm{g}^t$. Therefore, the model is defined by:
% \begin{enumerate}
% \item State Transition: $\bm{s}_{t+1} = f(\bm{s}^t, \bm{v}^t) $.
% \item Reward Function: $ \bm{r}(\bm{s}^t, \bm{a}^t) = g(\bm{s}^t, \bm{v}^t, \bm{g}^t) $.
% \end{enumerate}
% Here, functions $f$ and $g$ represent state transitions and reward calculations, respectively.
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{1204.png}
% %     \caption{Optimizer for RL implementation}
% %     \label{fig:optimizer}
% % \end{figure}

% Hence, we introduce an optimizer into our original mathodology. Following each state transmission in the MDP, the optimizer evaluates the newly transitioned state to determine the optimal combination of guard behaviors. Mathematically, this is expressed as:
% \[
% \bar{\bm{g}}^t = h(\bm{s}^{t+1} | \bm{s}^t, \bm{v}^t, f),
% \]
% where $\bar{\bm{g}}$ represents the optimal guard combination for the team, and $h$ is an optimizer function.

% Through the implementation of the optimizer, our original two-dimensional hybrid action space is effectively transformed into a one-dimensional continuous velocity space.

% \subsection{Hierarchical-CTDE}

% Although the optimizer reduces the action dimensionality and enhances computational efficiency, it assume the availability of global information. When implementing a decentralized approach, we encounter the challenge of relying on local observations due to communication constraints as $o^i^t \neq s^i^t$ for the $i$-th agent. Then, we formulate a framework of hierarchical centralized training and decentralized execution as shown in Fig.\ref{fig:H-CTDE}.

% During centralized learning, despite the communication barriers between agents, each agent's local observations are aggregated at a central processor. At this point, an optimizer is incorporated at the central unit to generate the team's optimal guard combination, which is then disseminated to the respective agents. Consequently, each agent's velocity behavior is produced by its corresponding actor network, while guard behaviors are allocated by the optimizer at the central processor. These behaviors are utilized to compute the reward for an actor-critic learning update process. 

% Within this framework, a 'policy' mechanism is introduced. Each agent is assigned a 'policy', which learns, through supervised learning, the agent's optimal guarding choice under varying local observations. These 'policies' form the intermediary layer of our learning architecture.

% During decentralized execution, although the central processor is no longer available, each agent can derive its velocity behavior from its own actor network. Additionally, the agent is informed of the guard choice it should make by its 'policy', thus facilitating the progression of the Markov Process.

% Such an architecture enables action dimensionality reduction even under conditions of communication constraints.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{CTDE2.pdf}
%     \caption{Hierarchical CTDE Framework}
%     \label{fig:H-CTDE}
% \end{figure}


%\section{mathod}




==> Contents_backup/conclusion.tex <==
\section{Conclusion}
% In this work, we introduced Bi-CL, a novel reinforcement learning framework designed to empower robots with the ability to learn complex coordination tasks through a bi-level optimization approach. Our methodology extends the centralized training and decentralized execution (CTDE) paradigm, addressing the inherent challenges of multi-robot systems, such as partial observability and the coupled nature of coordination behavior. 
We presented a bi-level formulation for multi-robot coordination learning with local observation, wherein robots' state transitions and their cooperative behaviors are abstracted and optimized on different levels, significantly enhancing learning efficiency. %We addressed the issue of mismatch between the centralized learning and decentralized execution in bi-level optimization due to the information loss. 
A key enabler of our Bi-CL algorithm was %We proposed an enhanced framework that incorporates 
an alignment penalty that enables upper-level learning to account for potential discrepancies arising from local observations in lower-level optimization. We validated our algorithm through a running example, designing two distinct environments: route-based and graph-based. Experimental results demonstrated that our algorithm can effectively learn in both environments, underscoring its versatility and applicability across a diverse set of coordination tasks. We evaluated the performance enhancement of the Bi-CL using different alignment penalty parameters. Comparative analysis with baselines verified the efficiency of our algorithm. 

For future work, we aim to explore the scalability of our Bi-CL to accommodate larger multi-robot systems and more complex environments, further refining the alignment penalty mechanism to enhance its adaptability and efficiency. Moreover, %considering our current algorithm's limitations in handling only fixed patterns of information loss due to local observations, 
we intend to extend our way of handling robots' information loss to effectively manage dynamic, stochastic, and noisy scenarios, thereby enhancing its resilience and performance in unpredictably evolving multi-robot coordination environments.

==> Contents_backup/intro.tex <==
\section{Introduction}


%\marginXW{\color{red}Multi-robot coordination is a challenging problem; It can be solved by may methods, including a promising one: CTDE; CTDE is difficult to train; We leverage Bi-level optimization for CTDE.}

Multi-robot systems have extensive applications in various engineering fields, but their deployment relies on scalable algorithms that enable robots to make coordinated and sequential decisions using local observation~\cite{rizk2019cooperative}. 
To this end, Centralized Training with Decentralized Execution (CTDE)~\cite{lowe2017multi} emerges as a promising approach, offering a balanced framework for coordinating multiple robots through centralized learning processes that guide decentralized operational decisions. However, the effectiveness of CTDE faces significant challenges as the dimensionality of action spaces expands and each robot only has local observation of the system. These challenges complicate the training process and potentially impedes practical deployment.

In this context, we note that multi-robot cooperative missions often exhibit inherent hierarchical structures, allowing them to be decomposed into high-level and low-level tasks~\cite{yan2013survey}. For instance, rescue missions utilize teams of robots to search large or hazardous areas~\cite{queralta2020collaborative, xiao2017uav, xiao2021autonomous, liu2021team}, where a high-level planning task may focus on area coverage, and a low-level task may address navigation and obstacle avoidance. A similar scenario arises from warehouse automation~\cite{lian2022spatio}, where high-level tasks involve managing robot fleets for picking, packing, and sorting, and low-level tasks ensure precise and safe navigation in densely populated environments.
Nevertheless, in most cases, the decomposed problems are internally coupled by state dependence, which can not be solved independently. Bi-level optimization~\cite{liu2021investigating} presents a solution to this issue, with the capability of enhancing learning efficiency and stability while maintaining the explicit connections between the two levels of problems. However, despite the abundance of research on addressing such coupling in static optimization problems for both single-agent~\cite{biswas2019literature} or multi-agent~\cite{zhang2020bi} cases, there remains a scarcity of studies tailored for multi-agent reinforcement learning (MARL) under CTDE with robots' local observation. This gap motivates our research to develop new approaches that leverage the benefits of bi-level optimization for reinforcement learning applications in multi-robot systems, thereby enhancing their deployment efficiency across a variety of complex and dynamic environments.


%To address this, we can leverage the bi-level optimization which can improve learning efficiency and stability while still explicitly preserving the interconnections between the two levels of problems. While there have been extensive existing research investigating how to address such coupling for static singe-agent or multi-agent optimization problems, limited research considers how to tailor it to multi-robot reinforcement learning with local observation. 

%Moreover, in many practical multi-agent problems, such as automated vehicle platooning and robotic soccer, the dimensions of actions are large, but there is a certain correlation between actions and between actions and rewards. For these complex multi-agent problems, our work introduces a novel application of {\color{blue}XXX algorithm}, aiming to enhance training efficiency and performance by embedding the bi-level optimization within the CTDE framework to reduce the dimensionality of the action spaces.


%Multi-robot coordination is always a formidable challenge within the realm of autonomous systems, demanding optimal solutions for effective collaboration and task execution among robots. While numerous methods have been explored to address this complexity, Centralized Training with Decentralized Execution (CTDE) emerges as a promising approach, offering a balanced framework for coordinating multiple robots through centralized learning processes that guide decentralized operational decisions. However, the effectiveness of CTDE is significantly hampered as the dimension of action spaces increases, leading to training difficulties that can impede practical implementation. Moreover, in many practical multi-agent problems, such as automated vehicle platooning and robotic soccer, the dimensions of actions are large, but there is a certain correlation between actions and between actions and rewards. For these complex multi-agent problems, our work introduces a novel application of {\color{blue}XXX algorithm}, aiming to enhance training efficiency and performance by embedding the bi-level optimization within the CTDE framework to reduce the dimensionality of the action spaces.

\noindent\textbf{Statement of contribution:}
The contributions of this paper include 
(i) the formulation of a bi-level Decentralized Markov Decision Process (Dec-MDP) for multi-robot coordination; 
%(i) the formulation of a bi-level Partially Observable Markov Decision Process (POMDP) for multi-robot coordination; 
(ii) a Bi-level Coordination Learning (Bi-CL) framework with a novel alignment mechanism to integrate multi-agent reinforcement learning and imitation learning under the CTDE scheme; (iii) simulated experiments that verify the effectiveness of the proposed Bi-CL algorithm and a comparison with traditional MARL algorithms to solve multi-robot coordination tasks. 

\begin{figure}
    \centering
    \includegraphics[width=0.46\textwidth]{Figures/intro/IROS24_running_eg1.pdf}
  \caption{A running example for a firefighting scenario. Robots can simultaneously perform two actions: move (to where) and guard (which adversary). Team reward depends on the risk of fire, which is a coupled function of both actions.}
   \label{fig_example1}
\end{figure}
\noindent\textbf{Running Example:} As visualized in Fig. \ref{fig_example1}, we introduce an example throughout this paper to conceptualize and verify the proposed bi-level approach for learning multi-robot coordination. 
Consider multiple robots traversing an area with multiple adversaries. During their traversal, each robot suffers risk or damage from adversaries accumulated over time, if it enters their impact range. We use robots' states to represent their physical locations. Each robot has two decomposable actions: the action of \textit{move} and the action of \textit{guard}, which are performed simultaneously. 
The \textit{move} action changes the robot's locations in the environment. In each step, the relative positions of robots to adversaries determine a base risk the robot accumulates. The \textit{guard} is an additional action each robot can choose to perform against an adversary, which increases its own risk but reduces the risks that this adversary poses to other robots. 
Our goal is to minimize the accumulated risk and traveling time for all robots to arrive at a target position, given each robot only has local (partial) observation of the system. 

Depending on the weights in performance evaluation, the team may face trade-offs between strategies. For example, each robot may move along the shortest path to reach the target as soon as possible v.s. spending more time to form guard behaviors to reduce team risk. These strategies boil down to robots' interdependent decision-making regarding move (to where) and guard (which adversary) at each time step, making the problem non-trivial. 
On the other hand, as a key idea this paper highlights, the move and guard actions of robots in this scenario exhibit a hierarchical structure. This structure can be leveraged through a bi-level reformulation, which simplifies the problem's complexity while still characterizing the interdependencies between the robots' two types of actions.



The same scenario discussed above applies to a handful of applications for multi-robot coordination, such as firefighting considering fire as adversaries; battlefields considering enemy robots as adversaries; and team car racing or football games considering non-cooperative players as adversaries.


%The difficulty of the described example arises from the combinatorial nature of robots' actions in deciding where to go and which adversary to guard. 

%Our goal is to minimize the risk accumulated across the entire multi-robot team, given each robot only has local (partial) observation of the system. 

%The optimal guard action clearly depends on other robots' location and their move action, and the risk associated with each move in return depends on the choice of the guard. This interdependence allows a bi-level formulation of the problem, with our goal to minimize the risk accumulated across the entire multi-robot team, given each robot only has local (partial) observation of the system. 

%The described scenario applies to a handful of applications for multi-robot coordination, such as firefighting considering fire as adversaries; battlefields considering enemy robots as adversaries; and team car racing or football games considering non-cooperative players as adversaries. % {\color{red}[Zechen: add]}

%In our study, we introduce {\color{blue}two cases} that are similar to the challenges described above and justify the applications in multi-agent system. As shown in Fig. \ref{fig_example1}, consider multiple firefight agents traversing a room in fire with multiple adversaries. During their traversal, agents suffer accumulated risk from adversaries that are close to them. Each agent has two de-composable actions: move and guard. Move action changes the location of the robot. Guard performs as a suppression of fires and is an additional action each agent chooses to perform (or not) against an adversary, which will increase the risk of its own but will reduce the risks this adversary incurs to other agents. The goal is to minimize the agent accumulated over the entire multi-agent team. The described scenario applies to a handful of applications for multi-agent coordination, such as firefighting, where some robots might deploy countermeasures to quell flames to ensure safer passage for their peers, or battlefields, where some agents can provide suppressive fire for allies to mitigate threats posed by the enemy.

%{\color{blue} Manshi's case}


% is introduced to conceptualize the formulated problem and justify its applications in multi-robot systems.  
% Consider multiple robots traversing an area with multiple adversaries. During their traversal, robots suffer accumulated risk from adversaries that are close to them. Let the agents' states, $s^i_t$, represent their physical locations. Each agent has two decomposable actions: the action of moving, ${x}^i_t$, and the action of guarding, ${y}^i_t$. 
% The \textit{move} action ${x}^i_t$ changes the agent's state (its location in the environment towards the target). In each step, the relative position of the agent to adversaries also determines a base risk the agent accumulates. The \textit{guard} ${y}^i_t$ is an additional action each agent chooses to perform (or not) against an adversary, which will increase the risk of its own but will reduce the risks this adversary incurs to other agents. The goal is to minimize the risk accumulated over the entire multi-robot team. {\color{red}[Add figure about the example, remove notations]}



==> Contents_backup/literature.tex <==
\section{Literature Review}
%\marginXW{{\color{red}Bi-level optimization, POMDP problem.ND-POMDP}}

\subsection{MARL for Multi-Robot Coordination}
Reinforcement Learning (RL) has gained significant popularity for controlling robotic systems for complex tasks~\cite{kaelbling1996reinforcement}. Using RL for multi-robot systems faces the challenge of increased system dimension and the need for robots to make decisions based on local observations. Addressing these challenges has led to the development of the CTDE~\cite{lowe2017multi} learning scheme, which enables robots to cooperatively learn coordination strategies through centralized training, while the learned policies are local and, thus, can be deployed for decentralized execution.  Examples include MADDPG~\cite{lowe2017multi}, which extends the centralized Deep Deterministic Policy Gradient (DDPG) framework to multi-robot systems. A similar case applies to Proximal Policy Optimization (PPO) algorithm and its generalization MAPPO \cite{yu2022surprising}. While these approaches might be concerned with state dimensionality during centralized training, recent advances, such as Value-Decomposition Networks (VDN), can be leveraged to decompose the joint value function into individual value functions for each robot~\cite{sunehag2017value}. Building on this, QMIX further extends the framework, allowing for a more complex, state-dependent mixing of individual robot's value functions to learn coordinated behaviors~\cite{rashid2020monotonic}. %Another line of research similar to bi-level decomposition is the use of human demonstrations to 

These CTDE approaches often rely on end-to-end learning, which cannot leverage the hierarchical structures of robot actions considered in this paper. In addition, their performance and training efficiency may significantly degrade~\cite{gmytrasiewicz2005framework} if each robot's local observation covers only parts of the state space.
Such local observation leads to a Decentralized Markov Decision Process (Dec-MDP), whose complexity is NEXP-complete~\cite{bernstein2002complexity}. In this case, even a slight reduction in the state/action space can have a huge impact on the overall computational complexity.

%leading to  
%a partially observable Markov Decision Process (POMDP)~\cite{zhang2011coordinated}. 
%Given that all robots' observations cover complete system states, the whole system is a Decentralized Markov Decision Process (Dec-MDP), whose complexity is NEXP-complete~\cite{bernstein2002complexity}. In this case, even a slight reduction in the state/action space can have a huge impact on the overall computational complexity.
%i.e., when the underlying system is a multi-agent Dec-MDP~\cite{bernstein2002complexity}~\cite{zhang2011coordinated}.

%Multi-agent coordination and cooperation have gradually gained popularity as a research field: how to collaborate to maximize the overall reward or benefit of the entire multi-agent system (MAS)? Many multi-agent reinforcement learning algorithms have been proposed in MAS following the introduction of CTDE \cite{lowe2017multi}, many of which are also applicable to multi-robot coordination. MADDPG \cite{lowe2017multi} extends the DDPG framework to multi-agent environments, allowing agents to learn cooperative and competitive strategies through CTDE. Similarly, MAPPO \cite{yu2022surprising} is an extension of the Proximal Policy Optimization algorithm to multi-agent settings. VDN \cite{sunehag2017value} is proposed to simplify the coordination of multi-agent reinforcement learning by decomposing the joint value function into individual value functions for each agent. Meanwhile, QMIX \cite{rashid2020monotonic} extends VDN by allowing for a more complex, state-dependent mixing of individual agents' value functions to learn coordinated behaviors, while maintaining a CTDE paradigm. However, methods built on the CTDE commonly face the challenge that is effectively handling partial observability and limited communication among agents in decentralized execution, especially when the number of agents increases and the dimensions of actions expand. Additionally, these methods often require sophisticated coordination mechanisms to balance individual agent goals with the overall system objective, while ensuring that learned policies are robust and can be successfully transferred from training to execution in dynamically changing real-world environments.


\subsection{Bi-level Optimization}

%Bi-level optimization, in our context, reinforcement learning, typically refers to a hierarchical structure where there are two distinct levels of decision-making, each with its own objectives and possibly its own learning process. The upper level might make high-level decisions (e.g., setting goals or tasks for lower levels), while the lower level focuses on executing these decisions within a more immediate or detailed context (e.g., navigating to a location). These levels operate at different timescales or with different scopes of the environment.
Regarding state/action space reduction,
bi-level optimization is a hierarchical mathematical formulation where the solution of one optimization task is restricted by the solution set mapping of another task~\cite{liu2021investigating}.
In recent years, this technique has been incorporated with various machine learning methods for nested decision-making, including multi-task meta-learning~\cite{antoniou2018train}, neural architecture search~\cite{liu2018darts}, adversarial learning~\cite{pfau2016connecting}, and deep reinforcement learning~\cite{hong2020two}. The applications of these bi-level learning approaches span economics, management, optimal control, systems engineering, and resource allocation problems~\cite{fortuny1981representation,sinha2017review,mintz2018control,nisha2022bilevel}, with a comprehensive review by Liu et al.~\cite{liu2021investigating}. 
Corresponding to the scope of this paper, when solving multi-robot coordination problems, bi-level decomposition has been introduced~ \cite{zhang2020bi,zheng2022stackelberg} for actor-critic MARL to reduce the training burden of each level, thus improving the training efficiency and convergence. 
Le et al.~\cite{le2017coordinated} uses latent variables to introduce a mechanism similar to bi-level optimization that can significantly improve the performance of multi-agent imitation learning.

Nevertheless, a commonality among the mentioned works is the assumption that robots (agents) can access complete state information of the system.
In cases where each robot has only partial information, the incomplete information can lead to a mismatch between the optimal solutions on the two levels. This challenge has motivated our work to incorporate an alignment penalty in order to generalize the bi-level optimization concept under CTDE, taking into account robots' local observations. 



%Inspired by these applications, for MDP problems with multiple action dimensions, we propose that these actions be similarly divided into two levels, where the upper level determines the state transitions of agents, and the lower level influences the benefits these state transitions bring to the system. By incorporating such bi-level optimization approach, we aim to enhance the effectiveness of algorithms within the CTDE framework more efficiently.

%Bi-Level Actor-Critic for Multi-Agent Coordination\cite{zhang2020bi}
%assumes complete informaiton.

%review\cite{liu2021investigating}

%[A hybrid machine-learning and optimization method to solve bi-level problems]

%[Bi-level optimization of charging scheduling of a battery swap station based on deep reinforcement learning]

%[Bi-level actor-critic for multi-agent coordination]
% #############################Commented introduction
\begin{comment}
Recent advancements in multi-agent systems have illuminated the intricate dynamics of environments where agents must execute both continuous and discrete actions. This complexity is exemplified in a range of applications, each presenting unique challenges and opportunities for optimization. In automated truck platooning, autonomous trucks dynamically adjust their speed and make strategic decisions about platoon leadership or formation, with the overarching goal of enhancing fuel efficiency and travel time. Similarly, in robotic soccer, each robot must finely tune its movement while also making critical decisions such as passing, shooting, or defending, aiming to maximize goals scored and defensive success. The intelligent traffic system scenario demands traffic signals to regulate light durations while also deciding on traffic flow priorities, balancing the need for traffic throughput against waiting times. Lastly, in a multi-robot warehouse system, robots must navigate and select tasks efficiently to optimize operational processes and task completion rates. 

These diverse scenarios collectively highlight the necessity for sophisticated approaches in managing hybrid action spaces, where the coordination of continuous and discrete actions plays a pivotal role in the system's overall performance and efficiency.

Additionally, in such complex multi-agent systems, efficiently finding and deploying optimal strategies to each agent, especially under communication constraints, poses a significant challenge. 

In our paper, we first formulate this problem using Markov Decision Process (MDP) and propose the Discrete Optimizer to optimize the intricate hybrid action space. We introduce a Hierarchical Centralized Training with Decentralized Execution (CTDE) framework for learning and deployment under local observations. Subsequently, we validate the feasibility of our approach theoretically and demonstrate its effectiveness through simulations.
\end{comment}

% \section{Standard CTDE Process}
% In the CTDE framework, agents are trained on a centralized basis with access to the global state and then executed in a decentralized manner where each agent may only observe a local view of the environment. The centralized training phase typically involves learning a joint policy that maximizes the global cumulative reward. Mathematically, this is represented as:
% \begin{equation}
% \max_{\pi} \mathbb{E} \left[ \sum_{t=0}^{T} \gamma^t r(s_t, \mathbf{a}_t) \right]
% \end{equation}
% where $ \pi $ denotes the joint policy, $ \gamma $ is the discount factor, $ r(s_t, \mathbf{a}_t) $ is the reward function, $ s_t $ is the global state, and $ \mathbf{a}_t $ is the joint action at time $ t $.

% \section{Enhanced Decentralized Execution}
% During decentralized execution, agents must operate effectively without access to the global state. The challenge addressed in this paper is that agents require an additional action dimension $ a_2 $, beyond the action $ a_1 $ used for state transitions. This is formalized as follows:

% The state transition of the multi-agent system is defined as:
% \begin{equation}
% s_{t+1} = \mathcal{T}(s_t, a_{1,t})
% \end{equation}
% where $ \mathcal{T} $ represents the state transition function, and $ a_{1,t} $ is the action responsible for the state transition at time $ t $.

% The decentralized reward function, which takes into account the additional action $ a_2 $, is given by:
% \begin{equation}
% r'(s^i_t, a_{1,t}^i, a_{2,t}^i) = f(s^i_t, a_{1,t}^i, a_{2,t}^i)
% \end{equation}
% where $ r' $ is the modified reward function in the decentralized setting, $ s^i_t $ is the local state observed by agent $ i $, $ a_{1,t}^i $ is the action taken by agent $ i $ according to the centralized policy, and $ a_{2,t}^i $ is the additional action taken by agent $ i $ during decentralized execution.

==> Contents_backup/problem.tex <==
\section{Preliminaries and Problem Formulation}
\subsection{Formulation of a Bi-level Optimization }\label{sec_centralized_bi}
A regular centralized Markov Decision Process (MDP) can be defined by a tuple $(\mathcal{S}, \mathcal{A}, \mathcal{T}, \gamma, {R})$, including state, action, state transition, discount factor, and reward. The goal is to learn a policy $\pi: \mathcal{S}\to\mathcal{A}$ to maximize the expected cumulative reward over the task horizon $T$, i.e.,
\begin{align}
    \max_{\pi} \quad\underset{{\bm{a}}_t \sim \pi(\cdot|{\bm{s}}_t)}{\mathbb{E}}\left[\sum_{t=0}^T \gamma^t R_t\right],  
    \label{eq_c_prob}
\end{align}
where $\bm{a}_t\in\mathcal{A}$ and $\bm{s}_t\in\mathcal{S}$ are the action and state of the system at each step.

Let's assume the actions of the system can be decomposed as $\bm{a}_t=\{{\bm{x}}_t,{\bm{y}}_t\}\in{\mathcal{X}}\times {\mathcal{Y}}$, and the system's state transition depends only on action ${\bm{x}}_t$ such that $\mathcal{T}:\mathcal{S}\times{\mathcal{X}}\to\mathcal{S}$:
\begin{align}\label{eq_trans}
    \bm{s}_{t+1}=\mathcal{T}(\bm{s}_t, {\bm{x}}_t).
\end{align}
However, the reward function depends on both actions:
\begin{align}\label{eq_reward}
    {R}_t=U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t). 
\end{align}
If the structure of problem \eqref{eq_c_prob} satisfies \eqref{eq_trans} and \eqref{eq_reward}, it can be formulated into a bi-level problem:
\begin{subequations}\label{eq_c_prob2}
    \begin{align}\label{eq_bilevel}
    &\max_{\widehat\pi} \quad\underset{{\bm{x}}_t \sim \widehat\pi(\cdot|{\bm{s}}_t)}{\mathbb{E}}\left[\sum_{t=0}^T \gamma^t U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}^{*}_t({\bm{s}}_t,{\bm{x}}_t))\right], \\
    &~\text{s.t.}\qquad {\bm{y}}^{*}_t({\bm{s}}_t,{\bm{x}}_t)= \arg\max_{{\bm{y}}_t}U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t). \label{eq_opt_bara}
\end{align}
\end{subequations}
%\begin{align}\label{eq_optbara}
%    {\bm{y}}_t^{\star}= f({\bm{s}}_t,{\bm{x}}_t) = \arg\max_{{\bm{y}}_t}U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t),
%\end{align}

In this paper, we make the following assumption: 
\begin{assumption}\label{ass_1}
Problem \eqref{eq_bilevel} is complex such that $\widehat \pi$ is solved using a reinforcement learning (e.g. actor-critic method), whereas problem \eqref{eq_opt_bara} can be solved explicitly and be described as a mapping $f: \mathcal{S}\times {\mathcal{X}}\to{\mathcal{Y}}$.
% Suppose problem \eqref{eq_bilevel} is complex such that $\widehat \pi$ is solved using a reinforcement learning (e.g. actor-critic method). 
% Suppose problem \eqref{eq_opt_bara} is an explicit function of ${\bm{y}}_t$, which is directly solvable by a mapping 
% $f: \mathcal{S}\times {\mathcal{X}}\to{\mathcal{Y}}$.
\end{assumption}

The assumption can be justified by the fact that \eqref{eq_bilevel} is a planning problem involving state transitions and rewards for future $T$ steps, while \eqref{eq_opt_bara} only involves a one-step reward.

Under Assumption \ref{ass_1}, for the lower level problem \eqref{eq_opt_bara}, the optimal ${\bm{y}}^{*}_t$ is solvable from $f: \mathcal{S}\times {\mathcal{X}}\to{\mathcal{Y}}$, based on the current $\bm{s}_t$ and the choice of ${\bm{x}}_t$. Bringing this solution back to the upper level \eqref{eq_bilevel}, we only need to solve a reduced-dimension MDP defined by $(\mathcal{S}, {\mathcal{X}}, \mathcal{T}, \gamma, {R})$, to obtain a policy $\widehat \pi: \mathcal{S}\to {\mathcal{X}}$ that generates action ${\bm{x}}_t$. 
During implementation, the policy $\pi$ in problem \eqref{eq_c_prob} can be a composition of 
$\pi=\widehat \pi\circ f$. We learn the policy $\widehat \pi$ to generate ${\bm{x}}_t$ from ${\bm{s}}_t$, then use $f$ to generate ${\bm{y}}_t$ from $\{{\bm{s}}_t,{\bm{x}}_t\}$. Fig. \ref{fig_optimizer} provides a visualization of this bi-level mechanism builds on actor-critic reinforcement leaning.

%composing a policy $\widehat \pi: \mathcal{S}\to {\mathcal{X}}$ learned from reinforcement learning, and the mapping $f: \mathcal{S}\times {\mathcal{X}}\to\bar{\mathcal{A}}$ by solving an optimization problem. 

%Suppose the solution to \label{eq_optbara} is solvable whose solution is ${\bm{y}}_t^{\star}= f({\bm{s}}_t,{\bm{x}}_t)$


%$\widehat \pi: \mathcal{S}\to {\mathcal{X}}$ is a policy only generates action ${\bm{x}}_t$ with an optimal ${\bm{y}}_t^{\star}$. And the optimal ${\bm{y}}_t^{\star}$ is solvable from \eqref{eq_optbara}. Problem \eqref{eq_c_prob2} is called bi-level because the upper problem \eqref{eq_bilevel} can be solved using an MDP with \textit{reduced-dimension} action space, defined by $(\mathcal{S}, {\mathcal{X}}, \mathcal{T}, \gamma, {R})$. The solution of the lower problem 


%Specifically, for any state  $\bm{s}_t$ and action ${\bm{x}}_t$, we can determine the second action ${\bm{y}}_t$ by solving 

%where we assume the optimization mapping $f$ is directly solvable. Bring the optimizer back to \eqref{eq_reward}, one has
%\begin{align}\label{eq_rew_c}
%    {R}_t= U({\bm{s}}_t,{\bm{x}}_t,f({\bm{s}}_t,{\bm{x}}_t))
%\end{align}
%This allows us to solve problem \eqref{eq_c_prob} using an MDP with \textit{reduced-dimension} action space, defined by $(\mathcal{S}, {\mathcal{X}}, \mathcal{T}, \gamma, {R})$. Fig. \ref{fig_optimizer} provides a visualization of this bi-level mechanism. 

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{Figures/method/Algorithm_C.pdf}
  \caption{A Centralized Bi-level Optimization for RL.}
   \label{fig_optimizer}
\end{figure}

\subsection{Bi-level Formulation for Multi-robot Coordination Learning with Local Robot Observation}
In this paper, we generalize the bi-level formulation into a multi-robot system with local observation. Consider a multi-robot system with a set of  $\mathbf{n}=\{1,\cdots,n\}$ robots. Suppose the centralized actions and states in \eqref{eq_c_prob} are decomposed into each robot's state and action as $\bm{s}_t = \{s^1_t, \dots, s^n_t\}\in \mathcal{S}$ and $\bm{a}_t = \{a^1_t, \dots, a^n_t\}\in\mathcal{A}$. Assume each robot's action can be further written as $a^i_t = \{{x}^i_t, {y}^i_t\}$, where the action ${x}^i_t$ determines the robot's local state update ${s}^i_{t+1}=\mathcal{T}^i({s}^i_t, {x}^i_t)$.
The multi-robot system shares a global reward determined by all robots' states, and their two actions: ${R}_t=U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t)$.

%The multi-robot version of the problem can still be solved by the centralized approach described in the above section. However, 

For many real-world applications, the deployment of a multi-robot system faces communication and sensing constraints, where each agent may only have access to the states of its neighbors through a network, denoted by set $\mathcal{N}_i$. The neighbors' states are a subset of the full system state, denoted by ${s}^{\mathcal{N}_i}_t\subsetneq {\bm{s}}_t$. 
%To characterize this, let $\bm{o}_{t}=\{o^1_t, \dots, o_n^t\} \in \mathcal{O}$ be the observation set at time $t$ with $\mathcal{O}$ being the observation space for all agents.
Such local observation turns the problem into a Dec-MDP. Under this constraint, the \textbf{problem of interest} in this paper is to learn a \textit{local} policy $\pi^i$ for each agent such that:
\begin{align}
    \max_{\pi^i} \quad\underset{{a}^i_t \sim \pi^i(\cdot|{s}^{\mathcal{N}_i}_t)}{\mathbb{E}}\left[\sum_{t=0}^T \gamma^t R_t\right]. 
    % \nonumber
    \label{eq_loca_prob}
\end{align}
%\marginXW{Check this formulation}
While solving Dec-MDP problems is known to be difficult~\cite{bernstein2002complexity}, in this paper, we will generalize the idea of bi-level optimization under the scheme of CTDE and use action space reduction to alleviate the challenges in high-dimensional parameter tuning for MARL.
Note that such a generalization is non-trivial and the main challenge lies in the local observation and local decision-making of each robot using incomplete information. As a consequence, compared with the centralized case, the robots cannot solve an optimization problem like \eqref{eq_opt_bara} to directly determine their secondary action $y^i_t$.

%can no longer be solved by incorporating a policy on reduced-dimension action space and an optimizer.
%This is due to the local observation and local decision-making of each robot, such that no centralized optimization problem like \eqref{eq_optbara} can be formulated to directly solve robots' secondary action ${\bm{y}}_t = \{\bar{a}^1_t, \dots, \bar{a}^n_t\}$.



%Then, our goal changes to learn a policy $\pi: \mathcal{O}\to\mathcal{A}$ from local observations:
%\begin{align}
%    \max_{\pi} \quad\underset{{\bm{a}}^t \sim \pi(\cdot|{\bm{o}}^t)}{\mathbb{E}}\left[\sum_{t=0}^T (\gamma)^t R^t\right]. 
    % \nonumber
%    \label{eqn::reward}
%\end{align}

%Our formulation is distinguished by two primary aspects: firstly, it contains a hybrid action space comprising two distinct dimensions of actions, one in the continuous domain and the other in the discrete domain. Secondly, the state transition depends solely on the continuous action, while the discrete action significantly influences the reward value.


\noindent\textbf{Running Example.} 
% is introduced to conceptualize the formulated problem and justify its applications in multi-robot systems.  
% Consider multiple robots traversing an area with multiple adversaries. During their traversal, robots suffer accumulated risk from adversaries that are close to them. Let the agents' states, $s^i_t$, represent their physical locations. Each agent has two decomposable actions: the action of moving, ${x}^i_t$, and the action of guarding, ${y}^i_t$. 
% The \textit{move} action ${x}^i_t$ changes the agent's state (its location in the environment towards the target). In each step, the relative position of the agent to adversaries also determines a base risk the agent accumulates. The \textit{guard} ${y}^i_t$ is an additional action each agent chooses to perform (or not) against an adversary, which will increase the risk of its own but will reduce the risks this adversary incurs to other agents. The goal is to minimize the risk accumulated over the entire multi-robot team. {\color{red}[Add figure about the example, remove notations]}
We demonstrate how formulation \eqref{eq_loca_prob} aligns with the running example. 
Let state ${s}_t^i$ represent robots' physical locations. The \textit{move} action is associated with ${x}^i_t$, which impacts the robots' state update. The \textit{guard} action is associated with ${y}^i_t$.
The risk function (negative reward) $U$ in each time step depends on the robots' current locations ${s}_t^i$, their move ${x}^i_t$, and how robots are guarding against adversaries, i.e., ${y}^i_t$.
Thus, the scenario satisfies \eqref{eq_trans}-\eqref{eq_reward} and can be reformulated into a multi-robot bi-level optimization problem. All robots only receive states from their neighbors ${s}^{\mathcal{N}_i}_t\subsetneq {\bm{s}}_t$, through an underlying network. %This is in line with our Dec-MDP formulation. 
% the following example of 
%multiple vehicles traversing an adversary-controlled area where agents 
%[Our goal is to minimize the overall cost of the team, which is determined by (i) accumulated risk when agents stay in adversary-impacted zones and (ii) mission completion time. During traversal, agents can reduce their speed and act as a `guard' (the slower, the better), which can decrease the risks certain adversary incurs. This leads to a trade-off between agents' guarding behaviors and their travel speeds. The formulated problem is highly non-convex and cannot be efficiently solved by existing algorithms.]
%can coordinate by suppressive fire from allies can mitigate threats posed by the enemy. Or multiple firefighters pass a fire-engulfed corridor, some members might deploy countermeasures to quell flames, ensuring safer passage for their peers.
%Consider a number of $n$ agents traversing in a path environment. The positions of agents are their states $s^i^t$. 
%Each agent has two actions $\{{x}^i_t=v^i_t, {y}^i_t=g^i_t\}$ where $v_t^i\in[0,v_{\max}]$ denote the velocity of the agent moving on the path thus impacts the state transition through a simple integrator 
% \begin{align}\label{eq_dyn}
%     s_{t+1}^i = s_t^i + v^i_t \Delta t.
% \end{align}
%The second action $g^i_t$ represents the guarding action. 
%Before agent $i$ arrives at the end of the path, each time-step will produce a time penalty, denoted by $P^i^t$. We define
%\begin{align}
%P^i^t = \begin{cases}p & \text{if}~ s^i^t < L,\\
%    0& \text{if} ~s^i^t = L.
%    \end{cases}
%\end{align}
%\noindent\textbf{Risk \& Guard(Reward):} Let $m$ denote the number of adversaries with each adversary located at $d_j\in [0, L]$. Suppose adversary $j$ possesses a unique impact zone, denoted by $\mathcal{M}_j$, which incurs costs on travel agents. 
%At time step $t$, if an agent is in this region, i.e., $s^i^t\in \mathcal{M}_j$, a cost $r_{i,j}^t$ will be incurred.
%During traversal, if $s_k^t\in\mathcal{M}_j$, agent $k\in\{1,\cdots,n\}$ can counteract adversary $j$ by reducing its speed and acting as a `guard'. 
%Specifically, let  $g^t_k\in\{1, 2,\cdots,m\}$ denote the index of the adversary that agent $k$ is guarding against at time $t$.
%Then, the risks that adversary $j$ incurs to agents $i,~\forall s^i^t \in \mathcal{M}_j$ are discounted to $\alpha_{k,j}^t r_{i,j}^t$, where
%is the discount factor with $\beta\in(0,1)$. When $v_k^t=0$, agent $k$ achieves best guarding performance $\alpha^t_{k,j}=1-\beta$, while as $v_k^t\to v_{\max}$, the guarding effect vanishes. Furthermore, we assume the guarding effects stack with each other, thus, considering all agents in the system guarding an adversary $j$, the risk it incurs to agent $i$ is discounted by all guards as
%    $\prod_{k=1}^n \alpha_{k,j}^t r_{i,j}^t$.
%Note that the guarding behavior leads to agents' coordination, as one agent can decrease its speed to benefit all traveling agents within the influence region of the guarded adversary. 
%Let \( r^t^i\in\{0, 1, 2,\cdots,m\} \) denote which adversary is being guarded by the \( i \)-th traveling agent at time \( t \), with $r^t^i=0$ meaning not guarding any adversary. 
%We have $ r^t^i=j $ only if \(s^i^t \in \mathcal{M}_{j}\), meaning that an agent esecuting a guarding action must be located within this influence region. 
%The effectiveness of the discount factor is influenced by the speed of the guarding agent. Let \(\mathcal{Z}_j^t\) be the set of agents satisfied the guarding action conditions. \(g_j(v_k^t)\) be the discount applied by the \(i\)-th traveling agent to the \(j\)-th adversary. \marginXW{You need to describe $g_j$.}
%Let \(\alpha^t_j\) be the discount factor applied on \(j\)-th adversary. The discount factor for the region is
%\begin{align}
%    \alpha^t_j = \prod_{k\in{\mathcal{Z}_j^t}} (1-g_j(v_k^t))
%\end{align} 
%\noindent{\textbf{Team Cost:}} 
%Let $T$ be the total time for all agents in the team to traverse the path.
%Based on the above definitions, the team cost considers the risks and time penalties accumulated by all agents,
%\begin{align}\label{eq_def_f}
%    \bm{J} = \sum_{i=1}^n (\bm{R}^i + \bm{P}^i),
%\end{align}
%where $\bm{R}^i = \sum_{t=1}^T R^i^t \Delta t$ and $\bm{P}^i = \sum_{t=1}^T P^i^t \Delta t.$ with
%\begin{align}\label{eq_def_Ri}
%    \quad R^i^t=\sum_{j=1}^m \prod_{k=1}^n \alpha_{k,j}^t r_{i,j}^t.
%\end{align}
%\noindent{\textbf{Problem of Interest:}} In each time step, agent $i$'s action is composed of %traveling speed $v_{i}^t$ and guard target $g^i^t$. To strategically design all agents' behaviors,
%let $\bm{v}^t = \{v_1^t, \dots, v_n^{t}\}$, and $\bm{g}^t = \{g_1^t, \dots, g_n^{t}\}$.
%The problem is to minimize the team cost, i.e., $t\in\{1,\cdots,T\}$
%\begin{align}
%    \min_{\{\bm{v}^t,\bm{g}^t\}} \bm{J}.
%\end{align}

==> Final/abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{abstract}
    In multi-robot systems, achieving coordinated missions remains a significant challenge due to the coupled nature of coordination behaviors and the lack of global information for individual robots.
    To mitigate these challenges, this paper introduces a novel approach, Bi-level Coordination Learning (Bi-CL), that leverages a bi-level optimization structure within a CTDE paradigm. Our bi-level reformulation decomposes the original problem into a reinforcement learning level with reduced action space, and an imitation learning level that gains demonstrations from a global optimizer. 
    % Both levels contribute to improved learning efficiency and scalability. We note that robots' incomplete information leads to mismatches between the two levels of learning models. To address this, 
    Bi-CL further integrates an alignment penalty mechanism, aiming to minimize the discrepancy between the two levels without degrading their training efficiency. We introduce a running example to conceptualize the problem formulation. Simulation results demonstrate that Bi-CL can learn more efficiently and achieve comparable performance with traditional multi-agent reinforcement learning baselines for multi-robot coordination.  



    
    %Bi-CL not only enhances learning efficiency but also maintains the intricate cooperative relationships between the execution of individual actions and group coordination behaviors. 
    
    
    %To mitigate the gap between the two levels of bi-level optimization due to incomplete information, Bi-CL further integrates an alignment penalty as a bridge between the two levels, aiming at minimizing the discrepancy and fostering better coordination and efficiency. We introduce a running example to conceptualize the problem formulation and apply Bi-CL to two variations of this example: route-based and graph-based scenarios. Simulation results demonstrate that Bi-CL can more efficiently learn and achieve comparable performance with traditional multi-agent reinforcement learning baselines for multi-robot coordination. 

    %To address these challenges, this paper introduces a novel approach, Bi-level Coordination Learning (Bi-CL).
    %Bi-CL is enabled by a bi-level optimization reformulation of multi-robot coordination within a centralized training and decentralized execution paradigm. One level of the problem is composed of a 
    
\end{abstract}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Final/approach.tex <==
\section{Main Approach}
%\marginXW{Worked till here}
%\subsection{CDET: Reinforcement learning + Imitation learning} 

%Given the characteristics \ref{eq_trans} \ref{eq_rew} of our formulation, it is evident that for each state transition, we need to optimize the discrete action to achieve the maximum reward under the known current state and the selected continuous action. Consequently, for the decision-making regarding the discrete action, upon knowing $\bm{s}^t$ and $\bm{a}_1^t$ at every step, incorporating a discrete optimizer, such as enumeration, dynamic programming, or greedy algorithms, enables us to find the optimal combination of $\bar{\bm{a}_2}^t$ under the given moment and conditions, which reads
%\begin{align}
%    \bar{\bm{a}_2}^t = f(\bm{s}^{t+1}) = f(\bm{s}^t, \bm{a}_1^t, \mathcal{T})
%\end{align}
%where, $\bar{\bm{a}_2}^t$ represents the optimal discrete action combination for the team, $f$ represents the discrete optimizer here. 

%By integrating a Discrete Optimizer, it effectively transforms the original multi-agent system from a two-dimensional hybrid action space into a one-dimensional continuous action space, which significantly enhances the efficiency of subsequent policy learning processes.

 %To address this, our idea is to train two local policies $$

%assumes the availability of global information. When implementing a decentralized approach, we encounter the challenge that each agent relies on local observations ${{s}}^{\mathcal{N}_i}_t \subsetneq {\bm{s}}_t$ to decide its actions. 
%We can employ a similar two-step mechanism, which first uses reinforcement learning to learn a local policy $\widehat \pi^i: \mathcal{S}^{\mathcal{N}_i}\to {\mathcal{X}}^i$ to determine ${\bm{x}}_t^i$ for each agent. However, in the second step, the local observation prohibits us from using an optimizer to generate the action ${\bm{y}}_t^i$ because it relies on global state and global action. %To address this, a feasible approach is to introduce another layer of reinforcement learning model to determine  $\widehat \eta^i: \mathcal{S}^{\mathcal{N}_i}\times {\mathcal{X}}^{\mathcal{N}_i}\to {\mathcal{Y}}^i$. However, since the global reward, c.f. \eqref{eq_rew_c}, rely on both action ${\bm{x}}_t,{\bm{y}}_t$, using two layers of coupled reinforcement learning results in poor convergence stability and low learning efficiency [x]. In some cases, it may even be less desirable than using reinforcement learning to learn ${\bm{x}}_t,{\bm{y}}_t$ simultaneously. 
%we will leverage the hierarchical action structure of the problem, and introduce a new approach (cf. Fig.\ref{fig_dist_optimizer}). The approach uses a reinforcement learning mechanism to determine $\widehat{\pi}^i$, and an imitation learning mechanism to learn a policy $\widehat \eta^i: \mathcal{S}^{\mathcal{N}_i}\times {\mathcal{X}}^{\mathcal{N}_i}\to {\mathcal{Y}}^i$. 



As described in Sec. \ref{sec_centralized_bi}, the centralized bi-level formulation leverages the optimizer \eqref{eq_opt_bara} to reduce the dimensionality of the action space, thereby enhancing training efficiency. However, such optimization requires global information, which is not accessible to robots during decentralized execution. Thus, robots cannot locally generate ${y_t^i}^{*}$.
To address this issue, in this section, we introduce a new reformulation to generalize the concept of bi-level optimization to a CTDE  setup. %{\color{red}[Add description of novelty?]}

%our approach employs a similar two-step mechanism and trains two local policies for each robot: one policy, $\widehat{\pi}^i: \mathcal{S}^{\mathcal{N}_i} \to \mathcal{X}^i$, generates $x^i_t$; another policy, ${\eta}^i: \mathcal{S}^{\mathcal{N}_i} \times \mathcal{X}^{\mathcal{N}_i} \to \mathcal{Y}^i$, generates actions $y^i_t$. We employ CTDE (Centralized Training with Decentralized Execution). With the help of a global optimizer, $\widehat{\pi}^i$ is trained using reinforcement learning with a reduced-action space. ${\eta}^i$ is trained using imitation learning, taking the global optimizer as an expert demonstration. Since the parameters of the two models are trained separately, we further introduce a penalty mechanism in the optimizer to ensure the alignment of the two policies.

To present our approach, we reformulate \eqref{eq_loca_prob} into the following Bi-level Coordination Learning (Bi-CL) problem, $\forall i\in\{1,\cdots,n\}$,
\begin{subequations}\label{eq_d_prob2}
    \begin{align}\label{eq_bilevel_d}
    &\max_{\widehat\pi^i} \quad\underset{{x}^i_t \sim \widehat\pi^i(\cdot|{s}^{\mathcal{N}_i}_t)}{\mathbb{E}}\left[\sum_{t=0}^T \gamma^t U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t))\right], 
    \\
    %&\min_{\eta^i} \quad\underset{{y}^i_t \sim \eta^i(\cdot|{s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)}{\mathbb{E}}\left[\mathcal{D}\big({y}^i_t,{{y}^i_t}^*(\bm{s}_t,{\bm{x}}_t)\big)\right]\label{eq_policy_bara_d}
    &\min_{\eta^i} \quad\underset{{y}^i_t \sim \eta^i(\cdot|{s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)}{\mathbb{E}}\|{y}^i_t - {{y}^i_t}^*(\bm{s}_t,{\bm{x}}_t)\|^2\label{eq_policy_bara_d}, 
    \\
    &\text{s.t.}~ {\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t)\!=\! \arg\max_{{\bm{y}}_t}\!\left[U({\bm{s}}_t\!,{\bm{x}}_t\!,{\bm{y}}_t) 
    \underbrace{-c_k \sum_{i=1}^{n}\mathcal{H}_i({y}^i_t, \eta^i))}_{\text{alignment penalty}}\right] \label{eq_opt_bara_d}
\end{align}
\end{subequations}
In equations \eqref{eq_bilevel_d} and \eqref{eq_policy_bara_d}, we aim to train two local policies for each robot: one policy, $\widehat{\pi}^i: \mathcal{S}^{\mathcal{N}_i} \to \mathcal{X}^i$, generates action $x^i_t$; another policy, ${\eta}^i: \mathcal{S}^{\mathcal{N}_i} \times \mathcal{X}^{\mathcal{N}_i} \to \mathcal{Y}^i$, generates action $y^i_t$.
Note that the two policies are coupled since their inputs rely on the outputs of each other. If training two policies simultaneously, such coupling can pose a stability issue and reduce training efficiency. To address this, our idea is to introduce a global optimizer \eqref{eq_opt_bara_d} under the CTDE scheme to decouple and guide the training of both policies, as we explain next and visualized in Fig. \ref{fig_dist_optimizer}.

%Firstly, equations \eqref{eq_bilevel_d} and \eqref{eq_opt_bara_d} represent a CTDE version of the bi-level problem \eqref{eq_c_prob2}. Temporarily ignore the penalty term. We introduce optimization problem \eqref{eq_opt_bara_d} to solve ${\bm{y}}_t^{\star}$. This solution is only used during the centralized training process and thus can utilize global information by aggregating all robots' states ${\bm{s}}_t$ and actions ${\bm{x}}_t$. Based on ${\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t))$, we train the local policy $\widehat\pi^i$ in \eqref{eq_bilevel_d} for each agent's ${{x}}^i_t$ using a \textit{reinforcement learning} scheme over a \textit{reduced-dimension} action space. 

\noindent\textbf{Bi-level optimization:} First, we introduce optimization problem \eqref{eq_opt_bara_d} to solve ${\bm{y}}_t^{\star}$. If temporarily ignoring the alignment penalty term, the equations \eqref{eq_bilevel_d} and \eqref{eq_opt_bara_d} together represent a CTDE version of the bi-level problem \eqref{eq_c_prob2}.  During the centralized training process, we can utilize global information for all robots' states ${\bm{s}}_t$ and actions ${\bm{x}}_t$ to solve ${\bm{y}}_t^{\star}$. Based on ${\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t)$, we train the local policy $\widehat\pi^i$ in \eqref{eq_bilevel_d} for each agent's ${{x}}^i_t$ using a \textit{reinforcement learning} scheme. $\widehat\pi^i$ has a \textit{reduced-dimension} action space because ${\bm{y}}_t^{\star}$ is not learned. 

On the other hand, while optimizer \eqref{eq_opt_bara_d} can be used in centralized training to obtain action ${\bm{y}}_t^{\star}$ for all robots, it cannot be used by robots during decentralized execution due to the local observations. Thus, we introduce \eqref{eq_policy_bara_d} to train a local policy $\eta^i$ to generate agent's ${{y}}^i_t$. The policy $\eta^i$ can be trained conveniently using an imitation learning (IL) scheme that uses optimizer \eqref{eq_opt_bara_d} as the \textit{expert demonstration}. 
%Here, a possible choice for the imitation loss $\mathcal{D}$ is 
%$$\mathcal{D}=\|{y}^i_t - {{y}^i_t}^*(\bm{s}_t,{\bm{x}}_t)\|,$$ 
Here, the imitation loss in \eqref{eq_policy_bara_d} measures the difference between the policy output ${y}^i_t$ using local information and the optimal action solved from optimizer \eqref{eq_opt_bara_d} using global information.


\begin{algorithm2e}[t]
\SetAlgoLined
% \KwResult{Trained Actor and Critic Networks}
 \textbf{Initialize} local RL models $\widehat{\pi}^i({s}^{\mathcal{N}_i}|\theta_{\widehat{\pi}^i})$ and IL models $\eta^i({s}^{\mathcal{N}_i}, x^{\mathcal{N}_i}|\theta_{\eta^i})$ for all robots. Initialize centralized critic $Q(\bm{s}, \bm{x}|\theta_Q)$ if needed;  \\
 \textbf{Initialize} alignment penalty co-efficient $c_k$;\\
 %\textbf{Initialize} step-size $\delta$ and replay buffer $\mathcal{B}$; \\
 %\textbf{Initialize} target networks $Q'$ and $\widehat{\pi}^{i'}$ with weights $\theta^{Q'} \leftarrow \theta^Q$ and $\theta^{\widehat{\pi}^{i'}} \leftarrow \theta^{\widehat{\pi}^i}$;\\
 \For{$\text{k} = 0$ \KwTo $T_k$}{
  %\textbf{Initialize} a random process $\mathcal{D}$, receive initial global state $\bm{s}_1$ and local observations ${\bm{s}}^{\mathcal{N}_i}_1$;\\
    Update coefficient $c_k=\frac{c}{1+e^{-\beta (k-h)}}$;\\
  \For{$t = 0$ \KwTo $T_t$}{
  \For{$i = 1$ \KwTo $n$}{
  Get action: $x^i_t$ by adding random perturbation to ${\widehat{\pi}^i}({s}^{\mathcal{N}_i}_t|\theta_{\widehat{\pi}^i})$;\\
   %Execute $x^i_t$;\\
   Get action: $\widehat{y}^i_t = \eta^i({s}^{\mathcal{N}_i}_t,{x}^i_t | \theta_{\eta^i})$;\\
   State update: ${s}^i_{t+1}=\mathcal{T}^i({s}^i_t, {x}^i_t)$;\\
   }
   Solve $\arg\max_{{\bm{y}}_t}\!\left[U(\bm{s}_t, \bm{x}_t, \bm{y}_t) 
    -c_k \sum_{i=1}^n\mathcal{H}_i\right]$ to obtain ${\bm{y}}_t^{\star}$;\\
   Observe reward $R_t = U(\bm{s}_t, \bm{x}_t, \bm{y}_t^{\star});$\\
   Record $(\bm{s}_t, \bm{x}_t, \bm{y}^{\star}_t, R_t, \bm{s}_{t+1})$ to a fixed size buffer $\mathcal{B}$ with first-in-first-out;\\
   Sample $(\bm{s}_{\tau}, \bm{x}_{\tau}, \bm{y}^{\star}_{\tau}, r_{\tau}, \bm{s}_{{\tau}+1})$ from $\mathcal{B}$ as a random minibatch of size $w$;\\
   Update critic network $\theta_{Q}$ using the minibatch, if critic exist;\\
   \For{$i = 1$ \KwTo $n$}{
    Update IL learning model $\theta_{\eta^i}$ using the minibatch;\\
    Update RL learning model: $\theta_{\widehat{\pi}^i}$ using the minibatch;
   }
   %Update each target network:\\
   %$\theta^{Q'} \leftarrow \tau\theta^Q + (1 - \tau)\theta^{Q'}$;\\
   %$\theta^{\widehat{\pi}^{i'}} \leftarrow \tau\theta^{\widehat{\pi}^{i}} + (1 - \tau)\theta^{\widehat{\pi}^{i'}}$;\\
  }
 }
 \caption{{The Bi-CL Algorithm}}
 \label{alg_1}
\end{algorithm2e}

\noindent\textbf{Alignment of the two policies:} We explain the alignment term in \eqref{eq_opt_bara_d}. Based on the above explanation, the policy $\widehat\pi^i$ is trained assuming the actions ${\bm{y}}_t^{\star}=\{{y^1_t}^*,\cdots,{y^n_t}^*\}$ are optimal for all robots, and the policy $\eta^i$ seeks to generate such optimal actions using only local information. Clearly, during decentralized execution, the optimality of $\eta^i$ can hardly be guaranteed, thus creating a mismatch between the policies $\widehat\pi^i$ and $\eta^i$. To address this, we introduce an alignment penalty term $c_k \sum_{i=1}^{n}\mathcal{H}_i({y}^i_t, \eta^i))$ in \eqref{eq_opt_bara_d}, where $c_k>0$ and
%$$\mathcal{H}_i=\|{y}^i_t-\mathbb{E}[\eta^i({s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)] \|$$ 
$$\mathcal{H}_i=\underset{\widehat{y}^i_t \sim \eta^i(\cdot|{s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)}{\mathbb{E}}\|{y}^i_t - {\widehat{y}^i_t}\|^2.$$ 
%\marginZC{$\widehat{y}^i_t=\eta^i(\cdot|{s}^{\mathcal{N}_i}_t,{x}^{\mathcal{N}_i}_t)$, ${\widehat{y}^i_t}$ is from the model}
Here, ${\widehat{y}^i_t}$ is the output of the model $\eta^i$, then $\mathcal{H}_i$ evaluates how well an action ${y}^i_t$ aligns with the policy $\eta^i$. Minimizing this penalty helps to reduce the mismatch between the two local policies. Mathematically, the value of $\mathcal{H}_i$ for each robot equals the loss in \eqref{eq_policy_bara_d}. Hence, $c_k$ is an important coefficient and we shall remark on its choice during the training. If $c_k \to 0$, the reformulation \eqref{eq_d_prob2} disregards the policy mismatch, always opting for the solution that maximizes $U$ to train $\widehat\pi^i$. 
Conversely, when $c_k\to \infty$, the penalty forces the training of $\widehat\pi^i$ using the action chosen by $\eta^i$, making the two policies fully coupled, and the IL \eqref{eq_policy_bara_d} no longer updates. 
To strike a balance, our idea is to make sure the IL model is sufficiently trained before the penalty is applied. For this purpose, we define a modified logistic function:
\begin{align}\label{eq_defck}
    c_k=\frac{c}{1+e^{-\beta (k-h)}}\quad \text{with}\quad c>0, \beta>0, h>0
\end{align}
where $k$ is the training episode. We let $c_k$ start with zero to `jump start' the training of $\widehat\pi^i$ and $\eta^i$ using the optimal ${\bm{y}}_t^{\star}$ for maximizing $U$. Afterwards, $c_k$ is gradually increased to a sufficiently large value $c$ to fine-tune $\widehat\pi^i$, taking into account the output of $\eta^i$ and ensuring alignment between the two policies, $\widehat\pi^i$ and $\eta^i$.
The described training scheme is summarized in Algorithm 1. 

% \begin{algorithm}[H]
% \SetAlgoLined
% % \KwResult{Trained Actor and Critic Networks}
% \textbf{Initialize} critic $Q(s, x, y|\theta^Q)$, actors $\widehat{\pi}^i(s|\theta^{\widehat{\pi}^i})$, target networks $Q'$, $\widehat{\pi}^{i'}$, replay buffer $R$, datasets $D^i$;\\
% \For{$\text{episode} = 1$ \KwTo $M$}{
%   Initialize random process $\mathcal{N}$, receive initial state $s_1$ and observations ${s}^{\mathcal{N}_i}_1$;\\
%   \For{$t = 1$ \KwTo $T$}{
%     \For{$i = 1$ \KwTo $n$}{
%       Select $x^i_t = {\widehat{\pi}^i}({s}^{\mathcal{N}_i}_t|\theta^{\widehat{\pi}^i}) + \mathcal{N}_t$, execute $x^i_t$, observe new state $s_{t+1}$, ${s}^{\mathcal{N}_i}_{t+1}$, reward $r_t$;\\
%     }
%     Store $(s_t, x_t, r_t, s_{t+1})$ in $R$, sample minibatch from $R$, compute target $y_j$, update critic, update actors, update target networks;\\
%   }
% }
% \For{$i = 1$ \KwTo $n$}{
%     \For{each data point in $D^i$}{
%         Construct $\eta_i$ using ${s}^{\mathcal{N}_i}_t, x^i_t$ to predict ${y^i_t}^*$:\\
%         \Indp Initialize $\eta_i$, determine best split, split dataset, recursively build tree, label leaves;\\
%         \Indm Evaluate $\eta_i$ on validation set;\\
%     }
% }
% \caption{Simplified DDPG and Decision Tree Training}
% \end{algorithm}

%\marginXW{what is $s_{\tau+1}$}
%\marginXW{Orders?}
%\marginXW{minibatch, where loops end?}
%\marginXW{why $Q'$}

\begin{comment}
\begin{algorithm}
\SetAlgoLined
% \KwResult{Trained Actor and Critic Networks}
 \textbf{Initialize} centralized critic $Q(s, x, y|\theta^Q)$, local actors $\widehat{\pi}^i({s}^{\mathcal{N}_i}|\theta^{\widehat{\pi}^i})$ and local policies $\eta^i({s}^{\mathcal{N}_i}, x^i|\theta^{\eta^i})$ for all robots \\
 \textbf{Initialize} coefficients $c_k=c(1-e^{-\beta t})$ and replay buffer $\mathcal{B}$; \\
 %\textbf{Initialize} target networks $Q'$ and $\widehat{\pi}^{i'}$ with weights $\theta^{Q'} \leftarrow \theta^Q$ and $\theta^{\widehat{\pi}^{i'}} \leftarrow \theta^{\widehat{\pi}^i}$;\\
 \For{$\text{episode} = 1$ \KwTo $T_e$}{
  \textbf{Initialize} a random process $\mathcal{D}$, receive initial global state $\bm{s}_1$ and local observations ${\bm{s}}^{\mathcal{N}_i}_1$;\\
  \For{$t = 1$ \KwTo $T$}{
  \For{$i = 1$ \KwTo $n$}{
   Select action $x^i_t = {\widehat{\pi}^i}({s}^{\mathcal{N}_i}_t|\theta^{\widehat{\pi}^i}) + \mathcal{N}_t$;\\
   Execute $x^i_t$;\\
   Get action $\widehat{y}^i_t = \eta^i({s}^{\mathcal{N}_i}_t,{x}^i_t | \theta^{\eta^i})$
   }
   Receive $(\bm{s}_{t+1}, {\bm{s}}^{\mathcal{N}_i}_{t+1})=\mathcal{T}(\bm{s}_t, \bm{x}_t)$;\\
   ${\bm{y}}_t^{\star}(\bm{s}_t,{\bm{x}}_t)\!=\! \arg\max_{{\bm{y}}_t}\!\left[U({\bm{y}}_t|{\bm{s}}_t,{\bm{x}}_t) 
    -c_k \sum_{i}\mathcal{H}_i\right]$;\\
   Receive optimal $\bm{y}_t$ combinations;\\
   Observe reward $r_t = U(\bm{s}_t, \bm{x}_t, \bm{y}_t^{\star})$\\
   Add $(\bm{s}_t, \bm{x}_t, \bm{y}^{\star}, r_t, \bm{s}_{t+1})$ to $\mathcal{B}$;\\
   Sample a random minibatch $(\bm{s}_{\tau}, \bm{x}_{\tau}, \bm{y}^{\star}, r_{\tau}, \bm{s}_{{\tau}+1})$ with size $W$ from $R$;\\
   \For{$i = 1$ \KwTo $n$}{
   Update each {\color{blue}optimizer policy} by minimizing the sample {\color{blue}optimizer policy} loss:\\
    $L^i_{{\color{blue}optimizer}} = - \frac{1}{W}\sum_{{\tau}} (y_{\tau}^{i\star}-\eta^i({s}^{\mathcal{N}_i}_{\tau},{x}^i_{\tau} | \theta^{\eta^i}))^2$
   }
   Set $z_{\tau} = r_{\tau} + \gamma Q'(\bm{s}_{{\tau}+1}, \bm{x}_{{\tau}+1}|\theta^{Q'})$ where $x^i_{{\tau}+1} = \widehat{\pi}^{i'}({s}^{\mathcal{N}_i}_{{\tau}+1}|\theta^{\widehat{\pi}^{i'}})$;\\
   Update critic by minimizing the critic loss where $L_{\text{critic}} = \frac{1}{W} \sum_{\tau} (z_{\tau} - Q(\bm{s}_{\tau}, \bm{x}_{\tau}|\theta^Q))^2$;\\
   \For{$i = 1$ \KwTo $n$}{
   Update each actor policy using the sampled policy gradient:\\
       $\nabla_{\theta^{\widehat{\pi}^i}} J \approx \frac{1}{N} \sum_{\tau} \nabla_{x_i} Q(\bm{s}, \bm{x}|\theta^Q)\nabla_{\theta^{\widehat{\pi}^i}} \widehat{\pi}^i({s}^{\mathcal{N}_i}|\theta^{\widehat{\pi}^i})|_{{s}^{\mathcal{N}_i}_{\tau}}$\\
    where in $Q(\bm{s}, \bm{x}|\theta^Q)$, ${\bm{s}=\bm{s}_{{\tau}}, x^i=\widehat{\pi}({s}^{\mathcal{N}_i}_{\tau})}$
   }
   Update each target network:\\
   $\theta^{Q'} \leftarrow \tau\theta^Q + (1 - \tau)\theta^{Q'}$;\\
   $\theta^{\widehat{\pi}^{i'}} \leftarrow \tau\theta^{\widehat{\pi}^{i}} + (1 - \tau)\theta^{\widehat{\pi}^{i'}}$;\\
  }
 }
 \caption{{Alg Name}}
\end{algorithm}
\end{comment}

\begin{comment}
\begin{remark}
    In the presentation of Algorithm \eqref{alg_1}, we assume the use of actor-critic-based methods for \eqref{eq_bilevel_d} and a quadratic mismatch function for the imitation loss \eqref{eq_policy_bara_d}. However, the proposed algorithm is also applicable to general CTDE setups when using other reinforcement learning and imitation learning methods. Furthermore, in handling the local observations of robots, there exist more advanced methods \cite[Sec. 2.2.2]{zhang2021multi} in the literature on Dec-MDPs and POMDPs that leverage the memory (historic states) of robots to learn more powerful policies. In this paper, we only use simple memory-less policies, but these more advanced methods are also compatible with Algorithm \eqref{alg_1}.
\end{remark}
\end{comment}

% \begin{algorithm2e}
%     \caption{XXX Algorithm}
%     \label{Alg_XXX}
%     \SetAlgoLined
%     Randomly \textbf{Initialize} critic network $Q(s, \widehat{a}, \bar{a}|\theta^Q)$ and actors $\mu_{i}(s|\theta^{\mu_{i}})$ with weights $\theta^Q$ and $\theta^{\mu_{i}}$;\\
%     \textbf{Initialize} target networks $Q'$ and $\mu_{i}'$ with weights $\theta^{Q'} \leftarrow \theta^Q, \theta^{\mu_{i}'} \leftarrow \theta^{\mu_{i}}$;\\
%     \textbf{Initialize} replay buffer $R$;\\
%     \textbf{Initialize} dataset $D^i$;\\
%     \For{episode = 1, M}{
%     \textbf{Initialize} a random process $\mathcal{N}$ for action exploration;\\
%     Receive initial global state $s_1$;\\
%     \For{t = 1, T}{
%     \For{i \in [1, n]}{
%     Select action $\widehat{a^it} = \mu(o^it|\theta^{\mu_{i}}) + \mathcal{N}_t$ according to the current policy and exploration noise;\\
%     Execute action $\widehat{a^it}$ and explore all possible $\bar{a^i}$ combinations;\\}
%     Observe reward $r_t$ and observe new global state $s_{t+1}$ and return the optimal combination $\bar{\bm{a}^i}$;\\
%     Store transition $(\bm{s}_t, \widehat{\bm{a}_t}, r_t, \bm{s}_{t+1})$ in $R$\;\\
%     Store data $(o^it, \widehat{a^it}, o_{t+1}, \bar{a^it})$ in $D^i$;\\
%     Sample a random minibatch of $N$ transitions $(\bm{s}_t, \widehat{\bm{a}_t}, r_t, \bm{s}_{t+1})$ from $R$;\\
%     \For{each sampled transition}{
%     Set $y_j = r_j + \gamma Q'(\bm{s}_{j+1}, \mu_1'(o_1_{j+1}, |\theta^{\mu_1'}), \mu_2'(o_2_{j+1}, |\theta^{\mu_2'}), \dots, \mu_n'(o_n_{j+1}, |\theta^{\mu_n'})|\theta^{Q'})$;\\
%     }
%     Update critic by minimizing the loss: $L = \frac{1}{N} \sum_j (y_j - Q(\bm{s}_j, \widehat{\bm{a}_j}|\theta^Q))^2$;\\
%     Update each actor policy using the sampled policy gradient:;\\
%     $\nabla_{\theta^{\mu^i}} J \approx \frac{1}{N} \sum_j \nabla_{\widehat{a}} Q(\bm{s}, \widehat{\bm{a}}|\theta^Q)|_{s=\bm{s}_j,\widehat{a}=\mu^i(o^ij)} \nabla_{\theta^\mu} \mu(s|\theta^\mu)|_{s_j}$;\\
%     }
%     }
% \end{algorithm2e}



%once ${\bm{x}}_t$ are determined, we can still utilize the optimizer $f: \mathcal{S}\times {\mathcal{X}}\to\bar{\mathcal{A}}$ to generate the team's optimal combination of the action ${\bm{y}}_t$. 


%As a consequence, we can not only learn a policy $\widehat \pi^i: \mathcal{S}\to {\mathcal{X}}$ for each agent to first determine action ${\bm{x}}_t$, then use an optimizer $f: \mathcal{S}\times {\mathcal{X}}\to\bar{\mathcal{A}}$ to generate the action ${\bm{y}}_t$

%despite the communication barriers between agents, each agent's local observations are aggregated at a central processor. At this point, an optimizer is incorporated at the central unit to generate the team's optimal combination of the discrete action $\bm{a}_2$, which is then disseminated to the respective agents. Consequently, each agent's continuous action $\bm{a}_1$ is produced by its corresponding actor network, while $\bm{a}_2$ are allocated by the optimizer at the central processor. These behaviors are utilized to compute the reward for an actor-critic learning update process. 

%Within this framework, a 'policy' mechanism is introduced. Each agent is assigned a 'policy', which learns, through supervised learning, the agent's optimal $\bm{a}_2$ choice under varying local observations. These 'policies' form the intermediary layer of our learning architecture.

%During decentralized execution, although the central processor is no longer available, each agent can derive its $\bm{a}_1$ from its own actor network. Additionally, the agent is informed of the $\bm{a}_2$ choice it should make by its 'policy', thus facilitating the progression of the Markov Process.

%Such an architecture enables action dimensionality reduction even under conditions of communication constraints.




% \subsection{Local Observation}

% The locality of observation needs to be considered due to multi-agent communication barriers. 

% Let $\delta_{ij}$ be the distance of $i$-th agent and $j$-th agent. Define $\Delta$ as the maximum distance for perfect communication between agents, such that if $\delta_{ij} \leq \Delta$, the state information of agents $i$ and $j$ can be communicated effectively, implying that agents $i$ and $j$ are aware of each other's position. Conversely, if $\delta_{ij} > \Delta$, communication between agents $i$ and $j$ is not possible, leading to a complete lack of state information exchange when the distance exceeds this threshold.

% In a multi-agent system, let $s_j^t$ represent the state of the $j$-th agent at time $t$. Then, the local observation of agent $i$, denoted as $o^i$, at time $t$ is defined by the set:
% \[
% o^i = \{ p_{ij} \cdot s_j^t | 1 \leq j \leq n \}
% \]
% where
% \[
% p_{ij} = \begin{cases} 
% 1 & \text{if } \delta_{ij} \leq \Delta, \\
% 0 & \text{otherwise}.
% \end{cases}
% \]

% \subsection{Optimizer}

% In the formulation, we define the action 'guard' as a team coordination behavior. Due to the presence of cooperative decision-making behavior, our action space is characterized as a hybrid one, encompassing both continuous and discrete domains. Specifically, the velocity behavior $v^i^t$ denotes the speed of the $i$-th agent at time $t$ in the continuous domain, while the guard behavior $g^i^t$ in the discrete domain represents the adversary guarded by the $i$-th agent at time $t$.

% In our MDP model, state transitions, denoted by $\bm{s}_{t+1}$, depend solely on the agents' velocity behaviors $\bm{v}^t$. However, the rewards, $\bm{r}(\bm{s}^t, \bm{a}^t)$, are determined by both velocity $\bm{v}^t$ and guard behaviors $\bm{g}^t$. Therefore, the model is defined by:
% \begin{enumerate}
% \item State Transition: $\bm{s}_{t+1} = f(\bm{s}^t, \bm{v}^t) $.
% \item Reward Function: $ \bm{r}(\bm{s}^t, \bm{a}^t) = g(\bm{s}^t, \bm{v}^t, \bm{g}^t) $.
% \end{enumerate}
% Here, functions $f$ and $g$ represent state transitions and reward calculations, respectively.
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{1204.png}
% %     \caption{Optimizer for RL implementation}
% %     \label{fig:optimizer}
% % \end{figure}

% Hence, we introduce an optimizer into our original mathodology. Following each state transmission in the MDP, the optimizer evaluates the newly transitioned state to determine the optimal combination of guard behaviors. Mathematically, this is expressed as:
% \[
% \bar{\bm{g}}^t = h(\bm{s}^{t+1} | \bm{s}^t, \bm{v}^t, f),
% \]
% where $\bar{\bm{g}}$ represents the optimal guard combination for the team, and $h$ is an optimizer function.

% Through the implementation of the optimizer, our original two-dimensional hybrid action space is effectively transformed into a one-dimensional continuous velocity space.

% \subsection{Hierarchical-CTDE}

% Although the optimizer reduces the action dimensionality and enhances computational efficiency, it assume the availability of global information. When implementing a decentralized approach, we encounter the challenge of relying on local observations due to communication constraints as $o^i^t \neq s^i^t$ for the $i$-th agent. Then, we formulate a framework of hierarchical centralized training and decentralized execution as shown in Fig.\ref{fig:H-CTDE}.

% During centralized learning, despite the communication barriers between agents, each agent's local observations are aggregated at a central processor. At this point, an optimizer is incorporated at the central unit to generate the team's optimal guard combination, which is then disseminated to the respective agents. Consequently, each agent's velocity behavior is produced by its corresponding actor network, while guard behaviors are allocated by the optimizer at the central processor. These behaviors are utilized to compute the reward for an actor-critic learning update process. 

% Within this framework, a 'policy' mechanism is introduced. Each agent is assigned a 'policy', which learns, through supervised learning, the agent's optimal guarding choice under varying local observations. These 'policies' form the intermediary layer of our learning architecture.

% During decentralized execution, although the central processor is no longer available, each agent can derive its velocity behavior from its own actor network. Additionally, the agent is informed of the guard choice it should make by its 'policy', thus facilitating the progression of the Markov Process.

% Such an architecture enables action dimensionality reduction even under conditions of communication constraints.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{CTDE2.pdf}
%     \caption{Hierarchical CTDE Framework}
%     \label{fig:H-CTDE}
% \end{figure}


%\section{mathod}




==> Final/conclusion.tex <==
\section{Conclusion}
% In this work, we introduced Bi-CL, a novel reinforcement learning framework designed to empower robots with the ability to learn complex coordination tasks through a bi-level optimization approach. Our methodology extends the centralized training and decentralized execution (CTDE) paradigm, addressing the inherent challenges of multi-robot systems, such as partial observability and the coupled nature of coordination behavior. 
We presented a bi-level formulation for multi-robot coordination learning with local observation, wherein robots' state transitions and their cooperative behaviors are abstracted and optimized on different levels, significantly enhancing learning efficiency. %We addressed the issue of mismatch between the centralized learning and decentralized execution in bi-level optimization due to the information loss. 
A key enabler of our Bi-CL algorithm was %We proposed an enhanced framework that incorporates 
an alignment penalty that enables upper-level learning to account for potential discrepancies arising from local observations in lower-level optimization. We validated our algorithm through a running example, designing two distinct environments: route-based and graph-based. Experimental results demonstrated that our algorithm can effectively learn in both environments, underscoring its versatility and applicability across a diverse set of coordination tasks. We evaluated the performance enhancement of the Bi-CL using different alignment penalty parameters. Comparative analysis with baselines verified the efficiency of our algorithm. 

For future work, we aim to explore the scalability of our Bi-CL to accommodate larger multi-robot systems and more complex environments, further refining the alignment penalty mechanism to enhance its adaptability and efficiency. Moreover, %considering our current algorithm's limitations in handling only fixed patterns of information loss due to local observations, 
we intend to extend our way of handling robots' information loss to effectively manage dynamic, stochastic, and noisy scenarios, thereby enhancing its resilience and performance in unpredictably evolving multi-robot coordination environments.

==> Final/intro.tex <==
\section{Introduction}


%\marginXW{\color{red}Multi-robot coordination is a challenging problem; It can be solved by may methods, including a promising one: CTDE; CTDE is difficult to train; We leverage Bi-level optimization for CTDE.}

Multi-robot systems have extensive applications in various engineering fields, but their deployment relies on scalable algorithms that enable robots to make coordinated and sequential decisions using local observation~\cite{rizk2019cooperative,wang2021distributed}. 
To this end, Centralized Training with Decentralized Execution (CTDE)~\cite{lowe2017multi} emerges as a promising approach, offering a balanced framework for coordinating multiple robots through centralized learning processes that guide decentralized operational decisions. A similar case applies to Proximal Policy Optimization (PPO) algorithm and its generalization Multi-agent PPO \cite{yu2022surprising}. While these approaches might be concerned with state dimensionality during centralized training, recent advances, such as Value-Decomposition Networks (VDN), can be leveraged to decompose the joint value function into individual value functions for each robot~\cite{sunehag2017value}. Building on this, QMIX~\cite{rashid2020monotonic} further extends the framework, allowing for a more complex, state-dependent mixing of individual robot's value functions to learn coordinated behaviors. However, the effectiveness of CTDE faces significant challenges as the dimensionality of action spaces expands and each robot only has local observation of the system. These challenges complicate the training process and potentially impedes practical deployment.
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/intro/IROS24_running_eg1.pdf}
  \caption{A running example for a firefighting scenario. Robots can simultaneously perform two actions: move (to where) and guard (which adversary). Team reward depends on the risk of fire, which is a coupled function of both actions.}
   \label{fig_example1}
   \vspace{-4ex}
\end{figure}

In this context, we note that multi-robot cooperative missions often exhibit inherent hierarchical structures, allowing them to be decomposed into high-level and low-level tasks~\cite{yan2013survey}. For instance, rescue missions utilize teams of robots to search large or hazardous areas~\cite{queralta2020collaborative, xiao2021autonomous}, where a high-level planning task may focus on area coverage, and a low-level task may address navigation and obstacle avoidance. A similar scenario arises from warehouse automation~\cite{lian2022spatio}, where high-level tasks involve managing robot fleets for picking, packing, and sorting, and low-level tasks ensure precise and safe navigation in densely populated environments.
Nevertheless, in most cases, the decomposed problems are internally coupled by state dependence, which can not be solved independently. Bi-level optimization~\cite{liu2021investigating} presents a solution to this issue, with the capability of enhancing learning efficiency and stability while maintaining the explicit connections between the two levels of problems. 

Bi-level optimization is a hierarchical mathematical formulation where the solution of one optimization task is restricted by the solution set mapping of another task~\cite{liu2021investigating}.
In recent years, this technique has been incorporated with various machine learning methods for nested decision-making, including multi-task meta-learning~\cite{antoniou2018train}, neural architecture search~\cite{liu2018darts}, adversarial learning~\cite{pfau2016connecting}, and deep reinforcement learning~\cite{hong2020two}. The applications of these bi-level learning approaches span economics, management, optimal control, systems engineering, and resource allocation problems~\cite{wang2022consensus,sinha2017review,mintz2018control,nisha2022bilevel,wang2019scalable}, with a comprehensive review by Liu et al.~\cite{liu2021investigating}. 
Corresponding to the scope of this paper, when solving multi-robot coordination problems, bi-level decomposition has been introduced~ \cite{zhang2020bi,zheng2022stackelberg} for actor-critic MARL to reduce the training burden of each level, thus improving the training efficiency and convergence. 
Le et al.~\cite{le2017coordinated} uses latent variables to introduce a mechanism similar to bi-level optimization that can significantly improve the performance of multi-agent imitation learning.

However, despite the abundance of research on addressing such coupling in static optimization problems for both single-agent~\cite{biswas2019literature,limbu2023team} or multi-agent~\cite{zhang2020bi} cases, there remains a scarcity of studies tailored for multi-agent reinforcement learning (MARL) under CTDE with robots' local observation. This gap motivates our research to develop new approaches that leverage the benefits of bi-level optimization for reinforcement learning applications in multi-robot systems, thereby enhancing their deployment efficiency across a variety of complex and dynamic environments.


%To address this, we can leverage the bi-level optimization which can improve learning efficiency and stability while still explicitly preserving the interconnections between the two levels of problems. While there have been extensive existing research investigating how to address such coupling for static singe-agent or multi-agent optimization problems, limited research considers how to tailor it to multi-robot reinforcement learning with local observation. 

%Moreover, in many practical multi-agent problems, such as automated vehicle platooning and robotic soccer, the dimensions of actions are large, but there is a certain correlation between actions and between actions and rewards. For these complex multi-agent problems, our work introduces a novel application of {\color{blue}XXX algorithm}, aiming to enhance training efficiency and performance by embedding the bi-level optimization within the CTDE framework to reduce the dimensionality of the action spaces.


%Multi-robot coordination is always a formidable challenge within the realm of autonomous systems, demanding optimal solutions for effective collaboration and task execution among robots. While numerous methods have been explored to address this complexity, Centralized Training with Decentralized Execution (CTDE) emerges as a promising approach, offering a balanced framework for coordinating multiple robots through centralized learning processes that guide decentralized operational decisions. However, the effectiveness of CTDE is significantly hampered as the dimension of action spaces increases, leading to training difficulties that can impede practical implementation. Moreover, in many practical multi-agent problems, such as automated vehicle platooning and robotic soccer, the dimensions of actions are large, but there is a certain correlation between actions and between actions and rewards. For these complex multi-agent problems, our work introduces a novel application of {\color{blue}XXX algorithm}, aiming to enhance training efficiency and performance by embedding the bi-level optimization within the CTDE framework to reduce the dimensionality of the action spaces.


\noindent\textbf{Statement of contribution:}
The contributions of this paper include 
(i) the formulation of a bi-level Decentralized Markov Decision Process (Dec-MDP) for multi-robot coordination; 
%(i) the formulation of a bi-level Partially Observable Markov Decision Process (POMDP) for multi-robot coordination; 
(ii) a Bi-level Coordination Learning (Bi-CL) framework with a novel alignment mechanism to integrate multi-agent reinforcement learning and imitation learning under the CTDE scheme; (iii) simulated experiments that verify the effectiveness of the proposed Bi-CL algorithm and a comparison with traditional MARL algorithms to solve multi-robot coordination tasks. 


\noindent\textbf{Running Example:} 
We conceptualize the proposed bi-level approach using an example, as visualized in Fig. \ref{fig_example1}.
%As visualized in Fig. \ref{fig_example1}, we introduce an example throughout this paper to conceptualize and verify the proposed bi-level approach for learning multi-robot coordination. 
Consider multiple robots traversing an area with multiple adversaries. During their traversal, each robot suffers risk or damage from adversaries accumulated over time, if it enters their impact range. 
% We use robots' states to represent their physical locations. 
Each robot has two decomposable actions: the action of \textit{move} and the action of \textit{guard}, which are performed simultaneously. 
The \textit{move} action changes the robot's locations in the environment. In each step, the relative positions of robots to adversaries determine a base risk the robot accumulates. The \textit{guard} is an additional action each robot can choose to perform against an adversary, which increases its own risk but reduces the risks that this adversary poses to other robots. 
Our goal is to minimize the accumulated risk and traveling time for all robots to arrive at a target position, given each robot only has local (partial) observation of the system.  

% Depending on the weights in performance evaluation, the team may face trade-offs between strategies. For example, each robot may move along the shortest path to reach the target as soon as possible v.s. spending more time to form guard behaviors to reduce team risk. These strategies boil down to robots' interdependent decision-making regarding move (to where) and guard (which adversary) at each time step, making the problem non-trivial. 
% On the other hand, as a key idea this paper highlights, the move and guard actions of robots in this scenario exhibit a hierarchical structure. This structure can be leveraged through a bi-level reformulation, which simplifies the problem's complexity while still characterizing the interdependencies between the robots' two types of actions.



The same scenario discussed above applies to a handful of applications for multi-robot coordination, such as firefighting considering fire as adversaries; battlefields considering enemy robots as adversaries; and team car racing or football games considering non-cooperative players as adversaries.


%The difficulty of the described example arises from the combinatorial nature of robots' actions in deciding where to go and which adversary to guard. 

%Our goal is to minimize the risk accumulated across the entire multi-robot team, given each robot only has local (partial) observation of the system. 

%The optimal guard action clearly depends on other robots' location and their move action, and the risk associated with each move in return depends on the choice of the guard. This interdependence allows a bi-level formulation of the problem, with our goal to minimize the risk accumulated across the entire multi-robot team, given each robot only has local (partial) observation of the system. 

%The described scenario applies to a handful of applications for multi-robot coordination, such as firefighting considering fire as adversaries; battlefields considering enemy robots as adversaries; and team car racing or football games considering non-cooperative players as adversaries. % {\color{red}[Zechen: add]}

%In our study, we introduce {\color{blue}two cases} that are similar to the challenges described above and justify the applications in multi-agent system. As shown in Fig. \ref{fig_example1}, consider multiple firefight agents traversing a room in fire with multiple adversaries. During their traversal, agents suffer accumulated risk from adversaries that are close to them. Each agent has two de-composable actions: move and guard. Move action changes the location of the robot. Guard performs as a suppression of fires and is an additional action each agent chooses to perform (or not) against an adversary, which will increase the risk of its own but will reduce the risks this adversary incurs to other agents. The goal is to minimize the agent accumulated over the entire multi-agent team. The described scenario applies to a handful of applications for multi-agent coordination, such as firefighting, where some robots might deploy countermeasures to quell flames to ensure safer passage for their peers, or battlefields, where some agents can provide suppressive fire for allies to mitigate threats posed by the enemy.

%{\color{blue} Manshi's case}


% is introduced to conceptualize the formulated problem and justify its applications in multi-robot systems.  
% Consider multiple robots traversing an area with multiple adversaries. During their traversal, robots suffer accumulated risk from adversaries that are close to them. Let the agents' states, $s^i_t$, represent their physical locations. Each agent has two decomposable actions: the action of moving, ${x}^i_t$, and the action of guarding, ${y}^i_t$. 
% The \textit{move} action ${x}^i_t$ changes the agent's state (its location in the environment towards the target). In each step, the relative position of the agent to adversaries also determines a base risk the agent accumulates. The \textit{guard} ${y}^i_t$ is an additional action each agent chooses to perform (or not) against an adversary, which will increase the risk of its own but will reduce the risks this adversary incurs to other agents. The goal is to minimize the risk accumulated over the entire multi-robot team. {\color{red}[Add figure about the example, remove notations]}



==> Final/literature.tex <==
\section{Literature Review}
%\marginXW{{\color{red}Bi-level optimization, POMDP problem.ND-POMDP}}

\subsection{MARL for Multi-Robot Coordination}
Reinforcement Learning (RL) has gained significant popularity for controlling robotic systems for complex tasks~\cite{kaelbling1996reinforcement}. Using RL for multi-robot systems faces the challenge of increased system dimension and the need for robots to make decisions based on local observations. Addressing these challenges has led to the development of the CTDE~\cite{lowe2017multi} learning scheme, which enables robots to cooperatively learn coordination strategies through centralized training, while the learned policies are local and, thus, can be deployed for decentralized execution.  Examples include MADDPG~\cite{lowe2017multi}, which extends the centralized Deep Deterministic Policy Gradient (DDPG) framework to multi-robot systems. A similar case applies to Proximal Policy Optimization (PPO) algorithm and its generalization MAPPO \cite{yu2022surprising}. While these approaches might be concerned with state dimensionality during centralized training, recent advances, such as Value-Decomposition Networks (VDN), can be leveraged to decompose the joint value function into individual value functions for each robot~\cite{sunehag2017value}. Building on this, QMIX further extends the framework, allowing for a more complex, state-dependent mixing of individual robot's value functions to learn coordinated behaviors~\cite{rashid2020monotonic}. %Another line of research similar to bi-level decomposition is the use of human demonstrations to 

These CTDE approaches often rely on end-to-end learning, which cannot leverage the hierarchical structures of robot actions considered in this paper. In addition, their performance and training efficiency may significantly degrade~\cite{gmytrasiewicz2005framework} if each robot's local observation covers only parts of the state space.
Such local observation leads to a Decentralized Markov Decision Process (Dec-MDP), whose complexity is NEXP-complete~\cite{bernstein2002complexity}. In this case, even a slight reduction in the state/action space can have a huge impact on the overall computational complexity.

%leading to  
%a partially observable Markov Decision Process (POMDP)~\cite{zhang2011coordinated}. 
%Given that all robots' observations cover complete system states, the whole system is a Decentralized Markov Decision Process (Dec-MDP), whose complexity is NEXP-complete~\cite{bernstein2002complexity}. In this case, even a slight reduction in the state/action space can have a huge impact on the overall computational complexity.
%i.e., when the underlying system is a multi-agent Dec-MDP~\cite{bernstein2002complexity}~\cite{zhang2011coordinated}.

%Multi-agent coordination and cooperation have gradually gained popularity as a research field: how to collaborate to maximize the overall reward or benefit of the entire multi-agent system (MAS)? Many multi-agent reinforcement learning algorithms have been proposed in MAS following the introduction of CTDE \cite{lowe2017multi}, many of which are also applicable to multi-robot coordination. MADDPG \cite{lowe2017multi} extends the DDPG framework to multi-agent environments, allowing agents to learn cooperative and competitive strategies through CTDE. Similarly, MAPPO \cite{yu2022surprising} is an extension of the Proximal Policy Optimization algorithm to multi-agent settings. VDN \cite{sunehag2017value} is proposed to simplify the coordination of multi-agent reinforcement learning by decomposing the joint value function into individual value functions for each agent. Meanwhile, QMIX \cite{rashid2020monotonic} extends VDN by allowing for a more complex, state-dependent mixing of individual agents' value functions to learn coordinated behaviors, while maintaining a CTDE paradigm. However, methods built on the CTDE commonly face the challenge that is effectively handling partial observability and limited communication among agents in decentralized execution, especially when the number of agents increases and the dimensions of actions expand. Additionally, these methods often require sophisticated coordination mechanisms to balance individual agent goals with the overall system objective, while ensuring that learned policies are robust and can be successfully transferred from training to execution in dynamically changing real-world environments.


\subsection{Bi-level Optimization}

%Bi-level optimization, in our context, reinforcement learning, typically refers to a hierarchical structure where there are two distinct levels of decision-making, each with its own objectives and possibly its own learning process. The upper level might make high-level decisions (e.g., setting goals or tasks for lower levels), while the lower level focuses on executing these decisions within a more immediate or detailed context (e.g., navigating to a location). These levels operate at different timescales or with different scopes of the environment.
Regarding state/action space reduction,
bi-level optimization is a hierarchical mathematical formulation where the solution of one optimization task is restricted by the solution set mapping of another task~\cite{liu2021investigating}.
In recent years, this technique has been incorporated with various machine learning methods for nested decision-making, including multi-task meta-learning~\cite{antoniou2018train}, neural architecture search~\cite{liu2018darts}, adversarial learning~\cite{pfau2016connecting}, and deep reinforcement learning~\cite{hong2020two}. The applications of these bi-level learning approaches span economics, management, optimal control, systems engineering, and resource allocation problems~\cite{fortuny1981representation,sinha2017review,mintz2018control,nisha2022bilevel}, with a comprehensive review by Liu et al.~\cite{liu2021investigating}. 
Corresponding to the scope of this paper, when solving multi-robot coordination problems, bi-level decomposition has been introduced~ \cite{zhang2020bi,zheng2022stackelberg} for actor-critic MARL to reduce the training burden of each level, thus improving the training efficiency and convergence. 
Le et al.~\cite{le2017coordinated} uses latent variables to introduce a mechanism similar to bi-level optimization that can significantly improve the performance of multi-agent imitation learning.

Nevertheless, a commonality among the mentioned works is the assumption that robots (agents) can access complete state information of the system.
In cases where each robot has only partial information, the incomplete information can lead to a mismatch between the optimal solutions on the two levels. This challenge has motivated our work to incorporate an alignment penalty in order to generalize the bi-level optimization concept under CTDE, taking into account robots' local observations. 



%Inspired by these applications, for MDP problems with multiple action dimensions, we propose that these actions be similarly divided into two levels, where the upper level determines the state transitions of agents, and the lower level influences the benefits these state transitions bring to the system. By incorporating such bi-level optimization approach, we aim to enhance the effectiveness of algorithms within the CTDE framework more efficiently.

%Bi-Level Actor-Critic for Multi-Agent Coordination\cite{zhang2020bi}
%assumes complete informaiton.

%review\cite{liu2021investigating}

%[A hybrid machine-learning and optimization method to solve bi-level problems]

%[Bi-level optimization of charging scheduling of a battery swap station based on deep reinforcement learning]

%[Bi-level actor-critic for multi-agent coordination]
% #############################Commented introduction
\begin{comment}
Recent advancements in multi-agent systems have illuminated the intricate dynamics of environments where agents must execute both continuous and discrete actions. This complexity is exemplified in a range of applications, each presenting unique challenges and opportunities for optimization. In automated truck platooning, autonomous trucks dynamically adjust their speed and make strategic decisions about platoon leadership or formation, with the overarching goal of enhancing fuel efficiency and travel time. Similarly, in robotic soccer, each robot must finely tune its movement while also making critical decisions such as passing, shooting, or defending, aiming to maximize goals scored and defensive success. The intelligent traffic system scenario demands traffic signals to regulate light durations while also deciding on traffic flow priorities, balancing the need for traffic throughput against waiting times. Lastly, in a multi-robot warehouse system, robots must navigate and select tasks efficiently to optimize operational processes and task completion rates. 

These diverse scenarios collectively highlight the necessity for sophisticated approaches in managing hybrid action spaces, where the coordination of continuous and discrete actions plays a pivotal role in the system's overall performance and efficiency.

Additionally, in such complex multi-agent systems, efficiently finding and deploying optimal strategies to each agent, especially under communication constraints, poses a significant challenge. 

In our paper, we first formulate this problem using Markov Decision Process (MDP) and propose the Discrete Optimizer to optimize the intricate hybrid action space. We introduce a Hierarchical Centralized Training with Decentralized Execution (CTDE) framework for learning and deployment under local observations. Subsequently, we validate the feasibility of our approach theoretically and demonstrate its effectiveness through simulations.
\end{comment}

% \section{Standard CTDE Process}
% In the CTDE framework, agents are trained on a centralized basis with access to the global state and then executed in a decentralized manner where each agent may only observe a local view of the environment. The centralized training phase typically involves learning a joint policy that maximizes the global cumulative reward. Mathematically, this is represented as:
% \begin{equation}
% \max_{\pi} \mathbb{E} \left[ \sum_{t=0}^{T} \gamma^t r(s_t, \mathbf{a}_t) \right]
% \end{equation}
% where $ \pi $ denotes the joint policy, $ \gamma $ is the discount factor, $ r(s_t, \mathbf{a}_t) $ is the reward function, $ s_t $ is the global state, and $ \mathbf{a}_t $ is the joint action at time $ t $.

% \section{Enhanced Decentralized Execution}
% During decentralized execution, agents must operate effectively without access to the global state. The challenge addressed in this paper is that agents require an additional action dimension $ a_2 $, beyond the action $ a_1 $ used for state transitions. This is formalized as follows:

% The state transition of the multi-agent system is defined as:
% \begin{equation}
% s_{t+1} = \mathcal{T}(s_t, a_{1,t})
% \end{equation}
% where $ \mathcal{T} $ represents the state transition function, and $ a_{1,t} $ is the action responsible for the state transition at time $ t $.

% The decentralized reward function, which takes into account the additional action $ a_2 $, is given by:
% \begin{equation}
% r'(s^i_t, a_{1,t}^i, a_{2,t}^i) = f(s^i_t, a_{1,t}^i, a_{2,t}^i)
% \end{equation}
% where $ r' $ is the modified reward function in the decentralized setting, $ s^i_t $ is the local state observed by agent $ i $, $ a_{1,t}^i $ is the action taken by agent $ i $ according to the centralized policy, and $ a_{2,t}^i $ is the additional action taken by agent $ i $ during decentralized execution.

==> Final/problem.tex <==
\section{Preliminaries and Problem Formulation}
\subsection{Formulation of a Bi-level Optimization }\label{sec_centralized_bi}
A regular centralized Markov Decision Process (MDP) can be defined by a tuple $(\mathcal{S}, \mathcal{A}, \mathcal{T}, \gamma, {R})$, including state, action, state transition, discount factor, and reward. The goal is to learn a policy $\pi: \mathcal{S}\to\mathcal{A}$ to maximize the expected cumulative reward over the task horizon $T$, i.e.,
\begin{align}
    \max_{\pi} \quad\underset{{\bm{a}}_t \sim \pi(\cdot|{\bm{s}}_t)}{\mathbb{E}}\left[\sum_{t=0}^T \gamma^t R_t\right],  
    \label{eq_c_prob}
\end{align}
where $\bm{a}_t\in\mathcal{A}$ and $\bm{s}_t\in\mathcal{S}$ are the action and state of the system at each step.

Let's assume the actions of the system can be decomposed as $\bm{a}_t=\{{\bm{x}}_t,{\bm{y}}_t\}\in{\mathcal{X}}\times {\mathcal{Y}}$, and the system's state transition depends only on action ${\bm{x}}_t$ such that $\mathcal{T}:\mathcal{S}\times{\mathcal{X}}\to\mathcal{S}$:
\begin{align}\label{eq_trans}
    \bm{s}_{t+1}=\mathcal{T}(\bm{s}_t, {\bm{x}}_t).
\end{align}
However, the reward function depends on both actions:
\begin{align}\label{eq_reward}
    {R}_t=U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t). 
\end{align}
If the structure of problem \eqref{eq_c_prob} satisfies \eqref{eq_trans} and \eqref{eq_reward}, it can be formulated into a bi-level problem:
\begin{subequations}\label{eq_c_prob2}
    \begin{align}\label{eq_bilevel}
    &\max_{\widehat\pi} \quad\underset{{\bm{x}}_t \sim \widehat\pi(\cdot|{\bm{s}}_t)}{\mathbb{E}}\left[\sum_{t=0}^T \gamma^t U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}^{*}_t({\bm{s}}_t,{\bm{x}}_t))\right], \\
    &~\text{s.t.}\qquad {\bm{y}}^{*}_t({\bm{s}}_t,{\bm{x}}_t)= \arg\max_{{\bm{y}}_t}U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t). \label{eq_opt_bara}
\end{align}
\end{subequations}
%\begin{align}\label{eq_optbara}
%    {\bm{y}}_t^{\star}= f({\bm{s}}_t,{\bm{x}}_t) = \arg\max_{{\bm{y}}_t}U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t),
%\end{align}

In this paper, we make the following assumption: 
\begin{assumption}\label{ass_1}
Problem \eqref{eq_bilevel} is complex such that $\widehat \pi$ is solved using a reinforcement learning (e.g. actor-critic method), whereas problem \eqref{eq_opt_bara} can be solved explicitly and be described as a mapping $f: \mathcal{S}\times {\mathcal{X}}\to{\mathcal{Y}}$.
% Suppose problem \eqref{eq_bilevel} is complex such that $\widehat \pi$ is solved using a reinforcement learning (e.g. actor-critic method). 
% Suppose problem \eqref{eq_opt_bara} is an explicit function of ${\bm{y}}_t$, which is directly solvable by a mapping 
% $f: \mathcal{S}\times {\mathcal{X}}\to{\mathcal{Y}}$.
\end{assumption}

The assumption can be justified by the fact that \eqref{eq_bilevel} is a planning problem involving state transitions and rewards for future $T$ steps, while \eqref{eq_opt_bara} only involves a one-step reward.

Under Assumption \ref{ass_1}, for the lower level problem \eqref{eq_opt_bara}, the optimal ${\bm{y}}^{*}_t$ is solvable from $f: \mathcal{S}\times {\mathcal{X}}\to{\mathcal{Y}}$, based on the current $\bm{s}_t$ and the choice of ${\bm{x}}_t$. Bringing this solution back to the upper level \eqref{eq_bilevel}, we only need to solve a reduced-dimension MDP defined by $(\mathcal{S}, {\mathcal{X}}, \mathcal{T}, \gamma, {R})$, to obtain a policy $\widehat \pi: \mathcal{S}\to {\mathcal{X}}$ that generates action ${\bm{x}}_t$. 
During implementation, the policy $\pi$ in problem \eqref{eq_c_prob} can be a composition of 
$\pi=\widehat \pi\circ f$. We learn the policy $\widehat \pi$ to generate ${\bm{x}}_t$ from ${\bm{s}}_t$, then use $f$ to generate ${\bm{y}}_t$ from $\{{\bm{s}}_t,{\bm{x}}_t\}$. 
% Fig. \ref{fig_optimizer} provides a visualization of this bi-level mechanism builds on actor-critic reinforcement leaning.

%composing a policy $\widehat \pi: \mathcal{S}\to {\mathcal{X}}$ learned from reinforcement learning, and the mapping $f: \mathcal{S}\times {\mathcal{X}}\to\bar{\mathcal{A}}$ by solving an optimization problem. 

%Suppose the solution to \label{eq_optbara} is solvable whose solution is ${\bm{y}}_t^{\star}= f({\bm{s}}_t,{\bm{x}}_t)$


%$\widehat \pi: \mathcal{S}\to {\mathcal{X}}$ is a policy only generates action ${\bm{x}}_t$ with an optimal ${\bm{y}}_t^{\star}$. And the optimal ${\bm{y}}_t^{\star}$ is solvable from \eqref{eq_optbara}. Problem \eqref{eq_c_prob2} is called bi-level because the upper problem \eqref{eq_bilevel} can be solved using an MDP with \textit{reduced-dimension} action space, defined by $(\mathcal{S}, {\mathcal{X}}, \mathcal{T}, \gamma, {R})$. The solution of the lower problem 


%Specifically, for any state  $\bm{s}_t$ and action ${\bm{x}}_t$, we can determine the second action ${\bm{y}}_t$ by solving 

%where we assume the optimization mapping $f$ is directly solvable. Bring the optimizer back to \eqref{eq_reward}, one has
%\begin{align}\label{eq_rew_c}
%    {R}_t= U({\bm{s}}_t,{\bm{x}}_t,f({\bm{s}}_t,{\bm{x}}_t))
%\end{align}
%This allows us to solve problem \eqref{eq_c_prob} using an MDP with \textit{reduced-dimension} action space, defined by $(\mathcal{S}, {\mathcal{X}}, \mathcal{T}, \gamma, {R})$. Fig. \ref{fig_optimizer} provides a visualization of this bi-level mechanism. 

%\begin{figure}
%    \centering
%    \includegraphics[width=.45\textwidth]{Figures/method/Algorithm_C.pdf}
%  \caption{A Centralized Bi-level Optimization for RL.}
%   \label{fig_optimizer}
%\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/method/Algorithm_D.pdf}
  \caption{A Bi-level Coordination Learning (Bi-CL) Algorithm: incorporating multi-agent reinforcement learning (MARL) and imitation learning (MAIL), guided by a global optimizer.} 
   \label{fig_dist_optimizer}
   \vspace{-4ex}
\end{figure}

\subsection{Bi-level Formulation for Multi-robot Coordination Learning with Local Robot Observation}
In this paper, we generalize the bi-level formulation into a multi-robot system with local observation. Consider a multi-robot system with a set of  $\mathbf{n}=\{1,\cdots,n\}$ robots. Suppose the centralized actions and states in \eqref{eq_c_prob} are decomposed into each robot's state and action as $\bm{s}_t = \{s^1_t, \dots, s^n_t\}\in \mathcal{S}$ and $\bm{a}_t = \{a^1_t, \dots, a^n_t\}\in\mathcal{A}$. Assume each robot's action can be further written as $a^i_t = \{{x}^i_t, {y}^i_t\}$, where the action ${x}^i_t$ determines the robot's local state update ${s}^i_{t+1}=\mathcal{T}^i({s}^i_t, {x}^i_t)$.
The multi-robot system shares a global reward determined by all robots' states, and their two actions: ${R}_t=U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t)$.

%The multi-robot version of the problem can still be solved by the centralized approach described in the above section. However, 

For many real-world applications, the deployment of a multi-robot system faces communication and sensing constraints, where each agent may only have access to the states of its neighbors through a network, denoted by set $\mathcal{N}_i$. The neighbors' states are a subset of the full system state, denoted by ${s}^{\mathcal{N}_i}_t\subsetneq {\bm{s}}_t$. 
%To characterize this, let $\bm{o}_{t}=\{o^1_t, \dots, o_n^t\} \in \mathcal{O}$ be the observation set at time $t$ with $\mathcal{O}$ being the observation space for all agents.
Such local observation turns the problem into a Dec-MDP. Under this constraint, the \textbf{problem of interest} in this paper is to learn a \textit{local} policy $\pi^i$ for each agent such that:
\begin{align}
    \max_{\pi^i} \quad\underset{{a}^i_t \sim \pi^i(\cdot|{s}^{\mathcal{N}_i}_t)}{\mathbb{E}}\left[\sum_{t=0}^T \gamma^t R_t\right]. 
    % \nonumber
    \label{eq_loca_prob}
\end{align}
%\marginXW{Check this formulation}
While solving Dec-MDP problems is known to be difficult~\cite{bernstein2002complexity}, in this paper, we will generalize the idea of bi-level optimization under the scheme of CTDE and use action space reduction to alleviate the challenges in high-dimensional parameter tuning for MARL.
Note that such a generalization is non-trivial and the main challenge lies in the local observation and local decision-making of each robot using incomplete information. As a consequence, compared with the centralized case, the robots cannot solve an optimization problem like \eqref{eq_opt_bara} to determine their secondary action $y^i_t$.

%can no longer be solved by incorporating a policy on reduced-dimension action space and an optimizer.
%This is due to the local observation and local decision-making of each robot, such that no centralized optimization problem like \eqref{eq_optbara} can be formulated to directly solve robots' secondary action ${\bm{y}}_t = \{\bar{a}^1_t, \dots, \bar{a}^n_t\}$.



%Then, our goal changes to learn a policy $\pi: \mathcal{O}\to\mathcal{A}$ from local observations:
%\begin{align}
%    \max_{\pi} \quad\underset{{\bm{a}}^t \sim \pi(\cdot|{\bm{o}}^t)}{\mathbb{E}}\left[\sum_{t=0}^T (\gamma)^t R^t\right]. 
    % \nonumber
%    \label{eqn::reward}
%\end{align}

%Our formulation is distinguished by two primary aspects: firstly, it contains a hybrid action space comprising two distinct dimensions of actions, one in the continuous domain and the other in the discrete domain. Secondly, the state transition depends solely on the continuous action, while the discrete action significantly influences the reward value.

\begin{comment}
\noindent\textbf{Running Example.} 
% is introduced to conceptualize the formulated problem and justify its applications in multi-robot systems.  
% Consider multiple robots traversing an area with multiple adversaries. During their traversal, robots suffer accumulated risk from adversaries that are close to them. Let the agents' states, $s^i_t$, represent their physical locations. Each agent has two decomposable actions: the action of moving, ${x}^i_t$, and the action of guarding, ${y}^i_t$. 
% The \textit{move} action ${x}^i_t$ changes the agent's state (its location in the environment towards the target). In each step, the relative position of the agent to adversaries also determines a base risk the agent accumulates. The \textit{guard} ${y}^i_t$ is an additional action each agent chooses to perform (or not) against an adversary, which will increase the risk of its own but will reduce the risks this adversary incurs to other agents. The goal is to minimize the risk accumulated over the entire multi-robot team. {\color{red}[Add figure about the example, remove notations]}
We demonstrate how formulation \eqref{eq_loca_prob} aligns with the running example. 
Let state ${s}_t^i$ represent robots' physical locations. The \textit{move} action is associated with ${x}^i_t$, which impacts the robots' state update. The \textit{guard} action is associated with ${y}^i_t$.
The risk function (negative reward) $U$ in each time step depends on the robots' current locations ${s}_t^i$, their move ${x}^i_t$, and how robots are guarding against adversaries, i.e., ${y}^i_t$.
Thus, the scenario satisfies \eqref{eq_trans}-\eqref{eq_reward} and can be reformulated into a multi-robot bi-level optimization problem. All robots only receive states from their neighbors ${s}^{\mathcal{N}_i}_t\subsetneq {\bm{s}}_t$, through an underlying network. %This is in line with our Dec-MDP formulation. 
% the following example of 
\end{comment}
%multiple vehicles traversing an adversary-controlled area where agents 
%[Our goal is to minimize the overall cost of the team, which is determined by (i) accumulated risk when agents stay in adversary-impacted zones and (ii) mission completion time. During traversal, agents can reduce their speed and act as a `guard' (the slower, the better), which can decrease the risks certain adversary incurs. This leads to a trade-off between agents' guarding behaviors and their travel speeds. The formulated problem is highly non-convex and cannot be efficiently solved by existing algorithms.]
%can coordinate by suppressive fire from allies can mitigate threats posed by the enemy. Or multiple firefighters pass a fire-engulfed corridor, some members might deploy countermeasures to quell flames, ensuring safer passage for their peers.
%Consider a number of $n$ agents traversing in a path environment. The positions of agents are their states $s^i^t$. 
%Each agent has two actions $\{{x}^i_t=v^i_t, {y}^i_t=g^i_t\}$ where $v_t^i\in[0,v_{\max}]$ denote the velocity of the agent moving on the path thus impacts the state transition through a simple integrator 
% \begin{align}\label{eq_dyn}
%     s_{t+1}^i = s_t^i + v^i_t \Delta t.
% \end{align}
%The second action $g^i_t$ represents the guarding action. 
%Before agent $i$ arrives at the end of the path, each time-step will produce a time penalty, denoted by $P^i^t$. We define
%\begin{align}
%P^i^t = \begin{cases}p & \text{if}~ s^i^t < L,\\
%    0& \text{if} ~s^i^t = L.
%    \end{cases}
%\end{align}
%\noindent\textbf{Risk \& Guard(Reward):} Let $m$ denote the number of adversaries with each adversary located at $d_j\in [0, L]$. Suppose adversary $j$ possesses a unique impact zone, denoted by $\mathcal{M}_j$, which incurs costs on travel agents. 
%At time step $t$, if an agent is in this region, i.e., $s^i^t\in \mathcal{M}_j$, a cost $r_{i,j}^t$ will be incurred.
%During traversal, if $s_k^t\in\mathcal{M}_j$, agent $k\in\{1,\cdots,n\}$ can counteract adversary $j$ by reducing its speed and acting as a `guard'. 
%Specifically, let  $g^t_k\in\{1, 2,\cdots,m\}$ denote the index of the adversary that agent $k$ is guarding against at time $t$.
%Then, the risks that adversary $j$ incurs to agents $i,~\forall s^i^t \in \mathcal{M}_j$ are discounted to $\alpha_{k,j}^t r_{i,j}^t$, where
%is the discount factor with $\beta\in(0,1)$. When $v_k^t=0$, agent $k$ achieves best guarding performance $\alpha^t_{k,j}=1-\beta$, while as $v_k^t\to v_{\max}$, the guarding effect vanishes. Furthermore, we assume the guarding effects stack with each other, thus, considering all agents in the system guarding an adversary $j$, the risk it incurs to agent $i$ is discounted by all guards as
%    $\prod_{k=1}^n \alpha_{k,j}^t r_{i,j}^t$.
%Note that the guarding behavior leads to agents' coordination, as one agent can decrease its speed to benefit all traveling agents within the influence region of the guarded adversary. 
%Let \( r^t^i\in\{0, 1, 2,\cdots,m\} \) denote which adversary is being guarded by the \( i \)-th traveling agent at time \( t \), with $r^t^i=0$ meaning not guarding any adversary. 
%We have $ r^t^i=j $ only if \(s^i^t \in \mathcal{M}_{j}\), meaning that an agent esecuting a guarding action must be located within this influence region. 
%The effectiveness of the discount factor is influenced by the speed of the guarding agent. Let \(\mathcal{Z}_j^t\) be the set of agents satisfied the guarding action conditions. \(g_j(v_k^t)\) be the discount applied by the \(i\)-th traveling agent to the \(j\)-th adversary. \marginXW{You need to describe $g_j$.}
%Let \(\alpha^t_j\) be the discount factor applied on \(j\)-th adversary. The discount factor for the region is
%\begin{align}
%    \alpha^t_j = \prod_{k\in{\mathcal{Z}_j^t}} (1-g_j(v_k^t))
%\end{align} 
%\noindent{\textbf{Team Cost:}} 
%Let $T$ be the total time for all agents in the team to traverse the path.
%Based on the above definitions, the team cost considers the risks and time penalties accumulated by all agents,
%\begin{align}\label{eq_def_f}
%    \bm{J} = \sum_{i=1}^n (\bm{R}^i + \bm{P}^i),
%\end{align}
%where $\bm{R}^i = \sum_{t=1}^T R^i^t \Delta t$ and $\bm{P}^i = \sum_{t=1}^T P^i^t \Delta t.$ with
%\begin{align}\label{eq_def_Ri}
%    \quad R^i^t=\sum_{j=1}^m \prod_{k=1}^n \alpha_{k,j}^t r_{i,j}^t.
%\end{align}
%\noindent{\textbf{Problem of Interest:}} In each time step, agent $i$'s action is composed of %traveling speed $v_{i}^t$ and guard target $g^i^t$. To strategically design all agents' behaviors,
%let $\bm{v}^t = \{v_1^t, \dots, v_n^{t}\}$, and $\bm{g}^t = \{g_1^t, \dots, g_n^{t}\}$.
%The problem is to minimize the team cost, i.e., $t\in\{1,\cdots,T\}$
%\begin{align}
%    \min_{\{\bm{v}^t,\bm{g}^t\}} \bm{J}.
%\end{align}

==> Final/results.tex <==
\section{Numerical Results}

In this section, we employ the running example to verify the proposed algorithm. We use simulated experiments to demonstrate: (i) the effectiveness of the proposed bi-level learning schemes, in particular, the alignment penalty term; (ii) the advantage of the proposed approach in terms of training efficiency compared with alternative MARL algorithms.


Through this section, we use the accumulated reward \eqref{eq_loca_prob} to evaluate the proposed Bi-CL algorithm. To avoid ambiguity, we distinguish the following metrics:

\noindent \textit{\textbf{RL-Reward}}: refers to the reward of the reinforcement learning policy $\widehat{\pi}^i$ when solving \eqref{eq_bilevel_d} during centralized training.

\noindent \textit{\textbf{T-Reward}}: refers to an average reward obtained by executing both the learned reinforcement learning policy $\widehat{\pi}^i$ and imitation learning policy $\eta_i$ in the environment for thirty times. 

\noindent \textit{\textbf{R-Gap}}: refers to the subtraction between the RL-Reward and the T-Reward.

\begin{remark}
    Note that RL-Reward and T-Reward are different because they use different ways to choose robots' action $y_t^i$. RL-Reward uses an `optimal' solution $\bm{y}_t^{\star}=\{{y^1_t}^{\star},\cdots, {y^n_t}^{\star}\}$ of \eqref{eq_opt_bara_d}; T-Reward uses output of the learned policy $\eta_i$. Only the T-Reward reflects the true performance of the policies because it is achievable during decentralized execution, and higher means better. Since R-Gap evaluates the difference, smaller means better.
\end{remark}



%we present simulated experiment results in two parts. (i) We demonstrate the necessity of the alignment penalty by conducting multiple experiments with different coefficients. Through these experimental results, we are able to select one suitable alignment penalty. (ii) We evaluate the performance of {\color{blue} XXX algorithm} combined with the popular MARL algorithms (MADDPG and VDN) on running example with different scenarios.

% \subsection{Coordinated Multi-robot Route Traversal}
%\marginXW{We need a thicker red-dash, anytime when zoom in/out, the red dashes are not visible.}
\begin{figure}[t]
    \vspace{-2ex}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/results/IROS24_running_ega.pdf}
    \caption{Running Example (a): all robots travel along a route.}
    \label{fig:example_a}
    \vspace{-3ex}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/results/IROS24_reward_ct_v3.pdf}
    \caption{Comparison of cumulative reward for different alignment penalties with four robots and four adversaries. The height of red dash lines determines implementation performance.}
    \label{fig:reward_ct}
    \vspace{-4ex}
\end{figure*}





\noindent\textbf{Running Example:}  We introduce a running example for coordinated multi-robot route traversal, by assuming all robots travel continuously through a route. Each robot can only observe a subset of full system states through an underlying communication network. Fig. \ref{fig:example_a} provides a visualization of the environment. The testing environment we use is a mathematical abstraction that may not exactly follow its physical layout and the number of adversaries may change.

\noindent~$\bullet$
Each robot $i$ has a continuous \textbf{\textit{move action}} (velocity) $x_t^i \in [-v_{\text{max}}, v_{\text{max}}]$, and a discrete \textbf{\textit{guard action}} $y_t^i \in\mathcal{M}$ where $\mathcal{M}$ is the set of all adversaries. The robot $i$'s \textbf{\textit{state transition}} (position) follows dynamics $s^i_{t+1}=s^i_{t}+x_t^i$. These align with definition \eqref{eq_trans}. 

\noindent~$\bullet$ 
Suppose adversary $j\in\mathcal{M}$ has an impacted area $\mathcal{B}_j$.
Each time-step, if $s^i_{t}\in\mathcal{B}_j$, robot $i$ accumulates a cost $c_j(s^i_{t})$. Besides, for any robot $k$, if $s^k_{t}\in\mathcal{B}_j$, it can perform guard against adversary $j$, i.e., $y^k_t=j$. The guarding effect is characterized by a discount factor on the costs created by adversary $j$:
\begin{align*}
    \alpha^{k,j}_t(x^k_t,y^k_t)=
    \begin{cases}
        1- \beta \frac{(v_{\max}-x^k_t)}{v_{\max}}& y^k_t=j,\\
        1&\text{otherwise}.
    \end{cases}
\end{align*}
Such a discount is more effective when the robot admits at a lower moving velocity $x_t^i$.
The total \textbf{\textit{team cost}} in each step is defined as: 
\begin{align*}
    R_t\!=\! U({\bm{s}}_t,{\bm{x}}_t,{\bm{y}}_t)\!=\!-\!\sum_{i=1}^n\!\sum_{j=1}^m \left[\prod_{k=1}^n \!\alpha^{k,j}_t\!(x^k_t,y^k_t)c^{i,j}_t(s^i_{t})\!\right]\!-\!\delta,
\end{align*}
where $\delta$ is a constant time penalty. A one-time positive reward is added when all robots arrive at the target. The definition of $U$ aligns with definition \eqref{eq_reward}.

\noindent~$\bullet$ The goal is to minimize the team accumulated cost in the form of \eqref{eq_loca_prob} before all robots arrive at the target position. 

The alignment of the problem with \eqref{eq_trans} and \eqref{eq_reward} allows it to be reformulated into \eqref{eq_d_prob2} and then solved by our Bi-CL. 

%\marginXW{LM methods explains.}

\begin{comment}
\begin{table}
    \centering
    \vspace{-1ex}
    \caption{Environment Configuration}

    \begin{tabular}{cc}
        \toprule
        \textbf{Parameter} & Value\\ \midrule 
        The length of path ($L$) & $50$  \\ \midrule
        Speed range ($V$) & $[0, 3]$  \\ \midrule
        Time penalty ($\delta$) & $0.1$  \\ \midrule
        Risk co-efficient ($\alpha$) & $1$  \\ \midrule
        Guard discount co-efficient ($\beta$) & $0.6$  \\ \midrule
        Reward reshape co-efficient ($c$) & $0.02$  \\ \midrule
        Stationary state penalty ($p$) & $1$  \\ \midrule
        Terminal state reward ($q$) & $100$  \\ \bottomrule
    \end{tabular}
    \label{table_env}
    \vspace{-1ex}
\end{table}
\end{comment}

%For the experiments, we adopt six scenarios denoted by \textit{Nx\_Mx} where \textit{N} represents the number of agents and \textit{M} represents the number of adversaries among the route. {\color{red} observation: homogeneous robots.
%And in scenario x, we reduce one more local observation dimension for all agents from originally $n-1$ to $n-2$. The general configuration of the running example is outlined in \ref{table_env}, which is consistent across all scenarios.}




\medskip
\noindent\textbf{Effectiveness of Alignment Penalty:} 
We first implement the proposed Bi-CL in an environment with 4 robots and 4 adversaries (fire). 
In Bi-CL, the reinforcement learning of $\widehat{\pi}^i$ uses an independent actor in each robot with centralized critic~\cite[Sec. 2.4]{xiao2022asynchronous}, following the structure of MADDPG~\cite{lowe2017multi} but over reduced action space.
%Each robot can observe the states of itself and two other robots, such that $\mathcal{N}_1=\{1,2,3\}$, $\mathcal{N}_2=\{2,3,4\}$, $\mathcal{N}_3=\{3,4,1\}$, $\mathcal{N}_4=\{4,1,2\}$. 
Each robot only observes part of the global information, i.e., its own state and the states of a subset of other robots in the system
The cost function $c_j$ is an affine function that depends on the closeness between the robot and the center of the adversary. 

Fig. \ref{fig:reward_ct} illustrates the RL-Reward curves and T-Reward for different $c_t$ by setting $c=0, c=1, c=5, c=10, c=50$, all with $\beta= 2e-3$ and $h=3000$. This, together with \eqref{eq_defck}, makes $c_k$ gradually increase in an `S' shape from $0$ to $c$. 
Upon examining the results, it is evident that the R-Gap is large when $c$ is small, and the gap diminishes as $c$ increases. This verifies the effectiveness of the proposed alignment penalty term in \eqref{eq_opt_bara_d}, as it motivates the policy $\widehat{\pi}_t^i$ to be tuned using a ${y_t^i}^{\star}$ that is closer to the output of $\eta_t^i$. 
It is also important to note that although the MARL training reward appears high when $c$ is small, this is misleading and unattainable in decentralized execution due to the mismatch between $\widehat{\pi}_t^i$ and $\eta_t^i$. The attainable reward (T-Reward) is much lower with smaller $c$.

\begin{table}[b]
    \centering
    \caption{Average reward per episode of different $c_k$ values}
    \small
    \setlength{\tabcolsep}{2.5pt} % Default value: 6pt, 3pt

    \begin{tabular}{ccccccc}
        \toprule
        \multirow{2}{*}{Environments} & \multirow{2}{*}{Metric} & \multirow{2}{*}{\(c_k=0\)} & \multicolumn{4}{c}{\(\beta=2e^{-3}\)}\\ 
         \cmidrule(rl){4-7} &  &  & \(c=1\) & \(c=5\)& \(\bm{c=10}\)& \(c=50\)\\
        \midrule 
        \multirow{2}{*}{\textit{N3\_M3}}
        & T-Reward & 51.83 & 53.01 & \textbf{53.44} & 53.17 & 52.13 \\
        & R-Gap & 1.34 & 0.73 & 0.26 & -0.45 & \textbf{-0.23} \\
        \midrule
        % \multirow{2}{*}{\textit{N3\_M3}}
        % & Ave. Rew & \textbf{54.81} & 52.01 & 51.74 & 54.75 & 53.62 \\
        % & Gap & -1.66 & -1.25 & -1.04 & \textbf{0.29} & 0.68 \\
        % \midrule
        % \multirow{2}{*}{\textit{N4\_M2}}
        % & Ave. Rew & 72.58 & \textbf{75.13} & 73.74 & 74.54 & 73.35 \\
        % & Gap & -2.9 & -1.83 & -1.3 & \textbf{-0.02} & 2.87 \\
        % \midrule
        \multirow{2}{*}{\textit{N4\_M4}}
        & T-Reward & 42.10 & 42.03 & 44.05 & \textbf{47.38} & {43.56} \\
        & R-Gap & 3.98 & 1.55 & -0.87 & -0.39 & \textbf{-0.11} \\
        \midrule
        \multirow{2}{*}{\textit{N5\_M4}}
        & T-Reward & 56.31 & 58.27 & 59.68 & \textbf{60.08} & 59.46 \\
        & R-Gap & 4.79 & 4.45 & 1.17 & \textbf{-0.04} & -0.15 \\
        \midrule
        \multirow{2}{*}{\textit{N5\_M4}*}
        & T-Reward & 50.67 & 53.39 & 54.09 & \textbf{54.60} & 54.20 \\
        & R-Gap & 6.54 & 3.84 & 1.82 & -0.59 & \textbf{0.27} \\
        \bottomrule
    \end{tabular}
    \label{table_results_cts}
\end{table}

Finally, we observe in the last plot of Fig. \ref{fig:reward_ct} that a very large $c=50$ may negatively impact the training performance. This is due to two reasons. First, as we discussed in the algorithm development, larger $c_k$ reduces the training efficiency of the imitation learning part of the algorithm. This is reflected by the lower values on both RL-Reward and T-Reward. 
Second, since $c_k$ impacts the computation of ${y_t^i}^{\star}$ during the training process, changing it too aggressively will lead to instability in training. This is evidenced by the middle part of the curve, where increased osculation is observed.

The same test is performed under various environment setups and the results are shown in Table \ref{table_results_cts}. Here, \textit{Na\_Mb} means the environment has $a$ robots and $b$ adversaries. %Each robot can observe the states of itself and $(a-2)$ other robots with a cyclic index similar to the above case. 
Especially, in \textit{N5\_M4*}, each robot further reduces the number of other robots's states it can observe. The results in the table align with our above analysis. In all cases where $c_k=c=0$, i.e., without alignment penalty, the performance is the worst. The R-Gap generally reduces when $c$ grows large. Since T-Reward is the core metric for performance, the best result mostly occurs at $c=10$ with only one exception and the difference is small.
Furthermore, to read the table column-wise, environments with the same number of adversaries, i.e., \textit{M4} are comparable. From \textit{N4\_M4} to \textit{N5\_M4}, the T-Rewards generally increase because more coordination behaviors can be generated. When comparing \textit{N5\_M4*} and \textit{N5\_M4}, the T-Rewards generally decrease due to the reduced sensing distances of the robots. This also leads to a larger R-Gap when $c=0$, necessitating the introduced alignment penalty.



%\marginXW{M3 or M5}

%As can be inferred from the graphs, under the same training conditions, the reward curve trends with the inclusion of a dynamic alignment penalty are largely consistent with one without an alignment penalty. This indicates that the setting of an alignment penalty does not affect the stability of the Actor-critic architecture. This constraint optimizes $\eta$ for mismatch correction without impacting the training of $\pi$. When we alter the magnitude of $c$, thereby adjusting the convergence upper limit of the alignment penalty, it is observed that an increase in $c$ leads to a gradual increase in the final average reward converging to levels close to, or even exceeding in the case of c=10, one without any penalty. {\color{red}However, as $c$ continues to increase, the training process becomes more turbulent. The observed turbulence in training with even higher $c$ values highlights a threshold beyond which the alignment penalty may introduce excessive volatility.}

%Additionally, to compare the performance, we executed agents' policies thirty times in the same test environment after training. Their performance is summarized in Tab. \ref{table_results_cts}. As for metrics in the table, the 'Ave. Rew' means the average reward obtained after thirty times' execution, employed to evaluate the actual test performance of the model post-training. While the 'Gap' represents the difference between the average reward after model inference and the expected reward value at convergence during the training process.The gap is utilized to observe the deviation in actual outcomes caused by mismatches generated during the training process. Tab. \ref{table_results_cts} shows that under our {\color{blue} BLHAC} framework, in the same scenario, it is observed that, in most cases, the comparisons of average rewards without penalties are lower than those with penalties though there is one exception in the simple scenario, i.e., \textit{N3\_M3}. In terms of gap comparisons, the absolute values of gaps with penalties are significantly smaller than those without penalties. {\color{red}Furthermore, a comparison under the same number of adversaries reveals that as the number of agents increases from 3 to 4 to 5, the rate of growth of the gap far exceeds that observed in the results with the alignment penalty since the sum of mismatch from $\eta_i$ is amplified by the increase of robots.} Based on the results from the table, we select a penalty logistic function when $c=10$ as a relatively optimal alignment penalty for subsequent comparisons with baseline algorithms since both the average reward and gap exhibit the best performance across the majority of scenarios under this condition. 

% In {\color{blue} BL-CTDE} framework, the results validate the existence of policy mismatch during the centralized training process, and this mismatch increases with the training episodes, causing the capability of model's decentralized execution to deviate progressively from the expected performance demonstrated during training.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{Figures/results/IROS24_algo.pdf}
%     \caption{Performance Comparison in Different Scenarios}
%     \label{fig:algo}
% \end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/results/iros24_reward_algo.pdf}
    \caption{Performance Comparisons in Different Scenarios.}
    \label{fig:algo}
    \vspace{-4ex}
\end{figure}

%\marginXW{(4) needs to be changed by running more trials. Why N5M4 converges bad, while N5M4* converges good. }

\medskip
\noindent\textbf{Comparing Training Efficiency with Baselines:} We also compare the proposed Bi-CL algorithm with two well-established MARL algorithms,  MADDPG~\cite{lowe2017multi} and QMIX~\cite{rashid2020monotonic}, respectively. MADDPG and QMIX are implemented in complete action space $\mathcal{A}^i=\mathcal{X}^i\times\mathcal{Y}^i$ of each robot. 
The same learning rates with Bi-CL are used. The comparison is visualized in Fig. \ref{fig:algo} for the four cases in the above discussion. Here, we choose $c=10$ as the R-Gaps are small. Thus, the RL-Reward curve can represent the convergence of our algorithm and can approximate the true reward our algorithm can achieve. It can be observed that in all cases, Bi-CL can achieve similar final rewards compared with baselines, which justifies the effectiveness of the proposed algorithm. The efficiency of Bi-CL is evidenced by its faster convergence speed compared with baselines. 
Furthermore, the starting reward of our algorithm is significantly better because it uses the optimization \eqref{eq_opt_bara_d} to boost and guide the policy training, while other methods are purely based on exploration.
For a similar reason, we observe that both MADDPG and QMIX suffer from training stability issues for complex scenarios, while the proposed Bi-CL does not. 



%In the second set of experiments, we primarily conducted a performance comparison between BLHAC and MADDPG, VDN—two well-established MARL algorithms applicable to our running example. We configured identical training parameters to train these three algorithms across six scenarios multiple times. The resulting learning curves are illustrated in Fig. \ref{fig:algo}, while a comparison of performance metrics during the training process is presented in Tab. \ref{table_results_alg}. We introduce the metric 'Converge' to represent the number of episodes at which the reward begins to converge, in order to compare the convergence speed of different algorithms. {\color{red}Convergence definition} {\color{blue}We identify the convergence by checking if the maximum difference of the moving rewards within a hundred window size falls below a threshold, indicating stability in performance}

%In Fig. \ref{fig:algo}, during the training process, since BLHAC solely explores $x$ to optimize $\eta$ related to $y$, it can achieve a relatively higher reward in the initial stages of training compared to MADDPG and VDN, which require exploration of both $x$ and $y$. {\color{red}Moreover, as the environment changes, BLHAC's adaptability to the environment is significantly stronger than that of MADDPG and VDN. MADDPG converges near a sub-optimal strategy when the number of robots is small. As the number of robots increases, VDN's training becomes highly unstable, experiencing a significant drop in reward during a period of episodes in the mid-training phase.} Coupled with Tab. \ref{table_results_alg}, we can observe that BLHAC not only converges to an optimal reward relatively smoothly during the training process but also demonstrates a superior convergence rate and onset in comparison to MADDPH and QMIX. This performance edge is attributed to BLHAC's innovative bi-level optimization. By leveraging bi-level optimization with alignment penalty, BLHAC ensures a more expedient and early convergence, thereby enhancing learning efficiency and effectiveness in complex scenarios. This distinct advantage underscores the potential of BLHAC in facilitating robust and agile solutions in the realm of cooperative multi-robot systems, where rapid adaptation and efficient policy learning are crucial.
% surpasses the other two algorithms in computational performance. Across different environments, with a comparable number of convergence iterations, BLHAC has a shorter average iteration time and lower CPU/GPU usage rates, significantly saving computational resources. This has very important implications for future applications to larger swarms of robots.


\begin{comment}
\subsection{Coordinated Multi-robot Graph Traversal}
\begin{figure}[h]
    \centering
    \vspace{-.5em}
    \includegraphics[width=0.45\textwidth]{Figures/results/IROS24_running_egb.pdf}
    \caption{Running Example (b): all robots travel through a graph.}
    \label{fig:example_b}
\end{figure}
\noindent\textbf{Running Example (b):} In the second scenario, we assume all robots travel through a graph environment, which highlights the coordination of robots from a spatial aspect. Fig. \ref{fig:example_b} provides a visualization of the environment; however, the testing environment we use includes randomly generated graphs that may not exactly follow the physical layout. Each robot can only observe a subset of full system states. The environment is characterized by a environment graph describing robot traversability from one node to another. It also features a coordination mechanism (green arrows) describing some robots, when located on certain nodes, can \textit{guard} other robots' edge traversal to reduce their cost, similar to the work by Limbu et al.~\cite{limbu2023team, limbuteam}.


\noindent~$\bullet$
Each robot $i$ has a discrete \textbf{\textit{move action}} $x_t^i\in\mathcal{N}(s^i_{t})$ that moves the robot to a new node in the graph based on its current position $s^i_{t}$. Here, $\mathcal{N}(s^i_{t})$ is the set of adjacent neighboring nodes of robot position  $s^i_{t}$ in the environment graph. The robot $i$'s \textbf{\textit{state transition}} (position) follows $s^i_{t+1}=x_t^i$ subject to $x_t^i\in\mathcal{A}(s^i_{t})$. 
The robot also has a discrete \textbf{\textit{guard action}} $y_t^i\in\mathcal{G}(x_t^i)$, where $\mathcal{G}(x_t^i)$ is the set of edges that can be guarded by a robot at its new position $s^i_{t+1}=x_t^i$ (visualized by green arrows in Fig. \ref{fig:example_b}).
The robots' actions and state transitions align with definition \eqref{eq_trans}.


\noindent~$\bullet$
When robot $i$ travels an edge $\{s^i_{t},x_t^i\}$, i.e., from $s^i_{t}$ to $s^i_{t+1}=x_t^i$, there is an associated edge cost $c(\{s^i_{t},x_t^i\})$. Besides, based on robot coordination, if another robot $k$ can and chooses to guard this edge, i.e., $y^k_t=\{s^i_{t},x_t^i\}\in\mathcal{G}(x_t^k)$, then this edge cost will be discounted by a factor 
\begin{align*}
    \alpha_t^{i,k}(s^i_{t},x_t^i,y^k_t)=
    \begin{cases}
    \alpha^* & y^k_t=\{s^i_{t},x_t^i\}\in\mathcal{G}(x_t^k),
    \\1 & \text{otherwise}.
    \end{cases}
\end{align*}
Based on this, the total \textbf{\textit{team cost}} in each step is defined as: 
\begin{align*}
    R_t\!= \!U({\bm{s}}_t,\!{\bm{x}}_t,\!{\bm{y}}_t)\!=\!-\!\!\sum_{i=1}^n \!\left[\prod_{k=1}^n \!\alpha_t^{i,k}(s^i_{t},x_t^i,y^k_t)c(\{s^i_{t},x_t^i\})\!\right] \!\!-\! \delta
\end{align*}
where $\delta$ is a constant time penalty. A one-time positive reward is added when all robots arrive at the target. The definition of $U$ aligns with definition \eqref{eq_reward}.

\noindent~$\bullet$ The goal is to minimize the team accumulated cost in the form of \eqref{eq_loca_prob} before all robots arrive at the target position. 

The alignment of the problem with \eqref{eq_trans} and \eqref{eq_reward} allows it to be reformulated into \eqref{eq_d_prob2} and then solved by our Bi-CL. 

\begin{table}[ht]
    \centering
    \caption{Comparison of Average Reward and Convergence time for Running Example (b)}
    \small
    \setlength{\tabcolsep}{2.5pt} % Default value: 6pt, 3pt

    \begin{tabular}{cccccccc}
        \toprule
        \multirow{ 2}{*}{Graph} & \multirow{ 2}{*}{\begin{tabular}{@{}c@{}}Robots/\\Nodes\end{tabular}}  & \multicolumn{3}{c}{T-Reward} & \multicolumn{3}{c}{Converge ($\times 10^3$)}\\
        \cmidrule(rl){3-5} \cmidrule(rl){6-8} & & Bi-CL & MAPPO & QMIX &  Bi-CL & MAPPO & QMIX \\
        \midrule 
        \multirow{4}{*}{Sparse} 
        & \textit{3/5}
        & \textbf{83.16} & 82.08 & 78.82 & \textbf{3.58} & 4.89 & 5.85 \\
        & \textit{3/10}
        & 64.86 & \textbf{65.39} & 64.97 & \textbf{3.69} & 4.87 & 5.95 \\
        & \textit{5/10}
        & 54.91 & 50.33 & \textbf{55.21} & \textbf{3.75} & 4.96 & 6.14 \\
        & \textit{5/15}
        & \textbf{51.37} & 33.14 & 49.67 & \textbf{3.71} & 5.24 & 6.03 \\
        \midrule
        \multirow{4}{*}{Dense}
        &\textit{3/5}
        & 93.21 & \textbf{96.90} & 94.23 & \textbf{3.63} & 4.95 & 6.19 \\
        & \textit{3/10}
        & \textbf{73.41} & 60.89 & 71.08 & \textbf{3.79} & 5.09 & 6.38 \\
        & \textit{5/10}
        & 66.32 & 54.14 & \textbf{68.08} & \textbf{3.80} & 4.94 & 6.29 \\
        & \textit{5/15}
        & \textbf{60.08} & 47.82 & 58.16 & \textbf{3.85} & 4.94 & 6.44 \\
        \bottomrule
    \end{tabular}
    \label{table_results_alg}
\end{table}


\medskip
\noindent\textbf{Comparing Training efficiency with Baselines:} In this scenario, we compare the proposed Bi-CL algorithm with two MARL algorithms MAPPO~\cite{lowe2017multi} and QMIX~\cite{rashid2020monotonic}, respectively. 
Here, we use MAPPO instead of MADDPG because %MADDPG cannot directly handle the discrete action in our graph-based coordination environment. Moreover, 
centralized PPO's suitability for this task has been validated by the study in Limbu et al.~\cite{limbuteam}.  
In Bi-CL, the reinforcement learning part is implemented by  QMIX in action space $\mathcal{X}_i$ for each robot. While the MAPPO and original QMIX are implemented in complete action space $\mathcal{A}^i=\mathcal{X}^i\times\mathcal{Y}^i$ of each robot. 
%In this running example, the action of each robot in our Bi-CL is determined by taking the argmax of each robot's Q value. The Q functions for each robot is updated by calculating the Temporal Difference (TD) error through the fitting of all Q functions into a global centralized Q function. 
The simulations are configured with the following setups. We experiment with 5, 10, 15 nodes in the environment graph with 3 or 5 robots in two types of graph connectivity, i.e., sparse and dense, for edges and the number of edges that can be guarded. We randomly create 15 environment graphs as our test set. For all approaches, training is terminated when the cumulative reward no longer changes more than $1\%$ for 10 steps. 

The comparison results are presented in Table \ref{table_results_alg}, which verifies the effectiveness of the Bi-CL algorithm for learning coordinated actions among robots within graph-based coordination tasks. Despite variations in the number of robots, graph nodes, or densities of the graph edges, the proposed Bi-CL algorithm delivers comparable results to the baseline algorithms while requiring fewer training episodes to converge. By observing the column of MAPPO, the results tend to fall below those of other methods under conditions of increased environmental complexity. This suggests that policy gradient approaches may only learn a sub-optimal policy solution in these cases.
The QMIX method is more robust in terms of optimality, however, it generally requires more training episodes to converge. In comparison, the proposed Bi-CL method enjoys much more efficient convergence properties. This improvement is mainly due to (i) the reduction of the action space for reinforcement learning, and (ii) the use of optimization \eqref{eq_opt_bara_d} to jump-start the training. 
\end{comment}


==> definitions.tex <==
\def\bs{\boldsymbol}
\def\mf{\mathbf}
\def\mb{\mathbb}
\def\mc{\mathcal}
\def\ms{\mathscr}
\def\beq{\begin{equation*}}
\def\eeq{\end{equation*}}
\def\bql{\begin{equation}}
\def\eql{\end{equation}}
\def\bqn{\begin{eqnarray*}}
\def\eqn{\end{eqnarray*}}
\def\bnl{\begin{eqnarray}}
\def\enl{\end{eqnarray}}

% \def\sgn{\text{sgn}}
\DeclareMathOperator{\sgn}{sgn} % this version ensures font matches things like \sin

% Agents
\newcommand{\att}[1]{$A_{#1}$}

% Speeds
\def\nufast{\nu_\text{fast}}
\def\nuslow{\nu_\text{slow}}
\def\nutrue{\nu}
\def\speed{v}

%==== Positions ====%
\def\x{\mf{x}}
\newcommand{\pos}[1]{\mf{x}_{#1}}
\newcommand{\vel}[1]{\mf{v}_{#1}}
\def\rai{r_{A_i}}
\def\raj{r_{A_j}}

%==== Angles ====%
\def\widthone{w_1}
\def\dang{\theta_{T}}
\def\Attackera{\theta_{A1}}  
\def\Attackerb{\theta_{A2}}
\def\angi{\theta_{A_i}}
\def\angj{\theta_{A_j}}

%==== Sets ====%
\def\reachone{\mc{R}_\text{1v1}}
\def\reachtwo{\mc{R}_\text{2v1}}
\def\thetaone{\Theta_\text{1v1}} 
\def\thetatwo{\Theta_\text{2v1}} 
\def\overlapone{\mc{I}_\text{1v1}} 
\def\overlaptwo{\mc{I}_\text{2v1}} 
\def\unionone{\mc{U}_\text{1v1}} 
\def\uniontwo{\mc{U}_\text{2v1}} 

\newcommand{\region}[1]{\Theta_{#1}}
\def\cone{\theta_{o1}}
\def\wone{w_{o1}}

%==== Strategies ====%
% \def\AttackerStrategy{\textbf{\color{black}``the strategy"}}
\def\AttackerStrategy{SS-FH strategy}

%==== Values ====%
\def\vone{V_\text{1v1}}
\def\vtwo{V_\text{2v1}}
\def\Runnercap{\tilde{\theta}}
